BeeGees: stayin' alive in chained BFT

Modern chained Byzantine Fault Tolerant (BFT) systems leverage a combination of pipelining and leader rotation to obtain both efficiency and fairness. These protocols, however, require a sequence of three or four consecutive honest leaders to commit operations. Therefore, even simple leader failures such as crashes can weaken liveness both theoretically and practically. Obtaining a chained BFT protocol that reaches decisions even if the sequence of honest leaders is non-consecutive, remains an open question. To resolve this question we present BeeGees, a novel chained BFT protocol that successfully commits blocks even with non-consecutive honest leaders. It does this while also maintaining quadratic word complexity with threshold signatures, linear word complexity with SNARKs, and responsiveness between consecutive honest leaders. BeeGees reduces the expected commit latency of HotStuff by a factor of three under failures, and the worst-case latency by a factor of seven.

==> podc_2022/evaluation.tex <==
\section{Evaluation}
%In our evaluation we answer three questions:
%\begin{enumerate}
%    \item What is the view change performance of Wendy \sys \xspace, and how does it compare to other protocols like 
%    Fast-HotStuff \sys s, SBFT \sys s, and Two-Chain HotStuff \sys s?
%    \item How much bandwidth does Wendy \sys s use compared to other \sys s?
%    \item How much additional key storage does Wendy \sys s need?
%\end{enumerate}

\natacha{To move to inside "implementation of aggregate signature scheme, as not a full evaluation?}
The previous section described the design of our new Oz aggregate signature scheme, with which we can efficiently implement no-commit proofs.  Through simulation, we quantitatively demonstrate the benefits of this approach in terms of performance, bandwidth and storage costs. In line with the goal of the paper, we focus on performance in the failure case for both leaders and follower replicas. All our experiments are run on a Cloudlab \textit{m510} machine (8-core 2.0 GHz CPU, 64 GB RAM, 10 GB, NIC). We compare against the approach taken by three representative protocols (described in Section~\ref{}). For fairness, we focus on \textit{chained} protocols that commit operations in two-phases in the non-failure case, and differ primarily in how they choose to implement their no-commit proof:
\begin{itemize}
    \item SBFT makes use of a linear number of \textit{BLS threshold} signatures
    \item Fast Hotstuff relies on a single \textit{BGLS signature}.
    \item Two-Chain Hotstuff sacrifices optimistic responsiveness to send a single \textit{BLS threshold signature} only, at the cost of waiting $\delta$. We set $\delta$ to 1 second as this is the default value chosen by the initial Two-Chain Hotstuff.
    \item Wendy, the protocol that we introduced in Section~\ref{}, requires a single Oz signature. 
\end{itemize}

\begin{center}
\begin{table*}[!t]
\caption{Communication Complexity of BFT protocols} %Overall Protocol Complexity - bit complexity, number of bits
% actually sent (excluding signatures), % authenticator complexity, number of signatures received or sent.
% Not every signature is created equal, some are more expensive than others, at one extreme, sending n signatures
% might be more expensive than sending n^2. 
% To understand this, need to look at table 1 and 2, 
% add Hotstuff, move responsiveness to table 3
% Need to look at theinvidiaul cryptographic costs of Table 1 and 2. Operations that are done are either
% group operations or pairings, so focus on those two metrics, and we look at it from two angles, what the
% leader has to do, and what the replicas have to do. Table 1 describes cost of leader verifying the new-view
% messages it received during the view change + time to generate any proof. 
\centering
\def\arraystretch{1.2}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
 \textbf{Protocol} & \makecell{\textbf{Bit Complexity}} & \makecell{\textbf{Authenticator Complexity}} &  \makecell{\textbf{Optimistic}\\\textbf{Responsiveness}} \\
 \hline
 Fast HotStuff & $O(n^3)$ & $O(n^2)$ & Yes \\ 
 SBFT~\cite{gueta2019sbft} & $O(n^2)$ & $O(n^2)$ & Yes \\ 
 Two-Chain HotStuff & $O(n)$ & $O(n)$ & No \\ 
 \textbf{Wendy} & $\mathbf{O(n^2 \log{n})}$ & $\mathbf{O(n)}$ & Yes \\
 \hline
\end{tabular}
\label{comparison}
\end{table*}
\end{center}

%\begin{center}
%\begin{table*}[!t]
%\caption{View Change Complexity of Leader in BFT protocols}
%\centering
%\def\arraystretch{1.2}
%\begin{tabular}{ |c|c|c|c|c| } 
% \hline
% \textbf{Protocol} & \makecell{\textbf{Pairing Complexity}} & \makecell{\textbf{Group Operation Complexity}} & \makecell{\textbf{Optimistic}\\\textbf{Responsiveness}} \\
% \hline%
%Fast HotStuff & $O(n)$ & $O(n^2)$ & Yes \\ 
% SBFT~\cite{gueta2019sbft} & $O(n)$ & $O(n)$ & Yes \\ %
% Two-Chain HotStuff & $O(n)$ & $O(n)$ & No \\ 
% \textbf{Wendy} & $\mathbf{O(n)}$ & $\mathbf{O(n^2)}$ & \textbf{Yes} \\
% \hline
%\end{tabular}
%\label{comparison}
%\end{table*}
%\end{center}

\begin{center}
\begin{table*}[!t]
\caption{Verification Cost}
\centering
\def\arraystretch{1.2}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
 \textbf{Signature Scheme} & \makecell{\textbf{Pairings}} & \makecell{\textbf{Multiplications}} \\
 \hline
 BLS threshold signatures & $O(1)$ & N/A \\ 
 BLS multi-signatures & $O(1)$ & $O(n)$ \\
 BGLS aggregate signatures & $O(n)$ & $O(n)$ \\ 
 \textbf{WendySig} & $\mathbf{O(1)}$ & $\mathbf{O(n \log{n})}$ \\
 \hline
\end{tabular}
\label{comparison}
\label{table:verification}
\end{table*}
\end{center}

\begin{center}
\begin{table*}[!t]
\caption{Signing Cost}
\centering
\def\arraystretch{1.2}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
 \textbf{Signature Scheme} & \makecell{\textbf{Exponentiations}} & \makecell{\textbf{Multiplications}} \\
 \hline
 BLS threshold signatures & $O(1)$ & N/A \\ 
 BLS multi-signatures & $O(1)$ & N/A \\
 BGLS aggregate signatures & $O(1)$ & N/A \\ 
 \textbf{WendySig} & $\mathbf{O(1)}$ & $\mathbf{O(\log{n})}$ \\
 \hline
\end{tabular}
\label{table:signing}
\end{table*}
\end{center}

\begin{center}
\begin{table*}[!t]
\caption{Aggregation Cost}
\centering
\def\arraystretch{1.2}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
 \textbf{Signature Scheme} & \makecell{\textbf{Multiplications}} \\
 \hline
 BLS threshold signatures & $O(n^2)$ \\ 
 BLS multi-signatures & $O(n)$ \\
 BGLS aggregate signatures & $O(n)$ \\ 
 \textbf{WendySig} & $\mathbf{O(n)}$ \\
 \hline
\end{tabular}
\label{table:aggregation}
\end{table*}
\end{center}


\begin{center}
\begin{table*}[!t]
\caption{Storage Costs for a single replica from different BFT protocols}
\centering
\def\arraystretch{1.2}
\begin{tabular}{ |c|c|c|c|c| } 
 \hline
 \textbf{Protocol} & \makecell{\textbf{Secret Keys}} & \makecell{\textbf{Public Keys}} & \makecell{\textbf{PoP}} \\
 \hline
 Fast HotStuff & $O(1)$ & $O(n)$ & $O(n)$ \\ 
 SBFT~\cite{gueta2019sbft} & $O(1)$ & $O(1)$ & N/A \\ 
 Two-Chain HotStuff & $O(1)$ & $O(1)$ & N/A \\ 
 \textbf{Wendy} & $\mathbf{O(n \log{n})}$ & $\mathbf{O(n^2 \log{n})}$ & $\mathbf{O(n^2 \log{n})}$ \\
 \hline
\end{tabular}
\label{table:storage}
\end{table*}
\end{center}


\begin{figure*}[!ht]
    \subfloat[100KB Batch Size]{{\includegraphics[width=5cm]{podc_figures/band-f.pdf}}}%
    \qquad
    \subfloat[f=333, n=1000]{{\includegraphics[width=5cm]{podc_figures/fhs-333.pdf} }}%
    \qquad
    \subfloat[f=333, n=1000]{{\includegraphics[width=5cm]{podc_figures/sbft-333.pdf} }}%
    \vspace{1em}
    \caption{Bandwidth as a function of batch size and scale}%
    \label{fig:band}%
\end{figure*}

\begin{figure*}[!ht]
    \subfloat[Key Storage]{{\includegraphics[width=5cm]{podc_figures/storage.pdf}}}%
    \qquad
    \vspace{1em}
    \subfloat[Leader Performance]{{\includegraphics[width=5cm]{podc_figures/proving.pdf}}}%
    \qquad
    \vspace{1em}
    \subfloat[Replica Performance]{{\includegraphics[width=5cm]{podc_figures/verification.pdf}}}%
    \qquad
    \vspace{1em}
    \caption{Storage and Performance as a function of scale}%
    \label{fig:storage}%
    
\end{figure*}

%\subsection{Experimental Setup}
%We run our experiments on a Cloudlab \textit{m510} machine (8-core 2.0 GHz CPU, 64 GB RAM, 10 GB, NIC). 

%We conduct
%a simulation study where we simulate the performance of the view change, bandwidth, and storage, as a function 
%of scale (number of replicas) and batch size.
%For experiments that are focused on scale, we simulate the local state of all the replicas, and measure performance 
%of the leader and a follower replica. 

%We quantity the cryptographic, network and storage costs of the view chan

\subsection{View Change Performance}
%For our first experiment we measure the simulated performance of the view changes of various BFT protocols. 
%We pick the three
%baselines of the Fast HotStuff, SBFT, and Two-Chain HotStuff, since they are representative of the different
%view change protocols. Note that the performance of these protocols are heavily influenced
%by the signature scheme that they use. Fast-HotStuff uses BLS multi-signatures and BGLS
%aggregate signatures, SBFT and Two-Chain HotStuff use BLS threshold signatures, and Wendy
%uses BlS multi-signatures and WendySig. We compare the performance of each signature scheme
%in tables 2-4.
%We measure the performance of Wendy, as a function of
%the number of replicas in the system and batch size. We divide the performance by leader and follower replica.
%We scale the number of replicas starting from $n=4$ 
%to $n=10000$ replicas. We show that Wendy has both low latency for both the leader and the follower replicas.
%
View-change costs can be split into proving latency at the leader (the time taken to generate the no-quorum proof), and verification latency at follower replicas
(time taken to verify proof validity).  We measure both as a function of number of participants and batch size.

\par \textbf{Leader proving time}. Figure~\ref{} measures proving time as a function of number of participants.
All protocols require that the leader verify $n-f$ \textsc{NewView} messages (each \textsc{NewView} message contains the highest QC each replica has seen .

In Fast-HotStuff, SBFT, and Two-Chain HotStuff, the leader 
verifies QCs from $n-f$ \textsc{NewView} messages it received. Each \textsc{NewView} message contains the highest QC
each replica has seen. For Two-Chain HotStuff
the leader must additionally wait $\Delta$ after receiving responses from $n-f$ replicas to ensure that it
receives responses from all honest replicas. Two-Chain HotStuff has $\approx 1s$ latency for $f<100$, since
$\Delta >> $ the time it takes to verify all of the \textsc{NewView} messages.
For $f=333$, SBFT and Two-Chain HotStuff have $9.3\%$ lower latency than Fast-HotStuff and Wendy, since SBFT
and Two-Chain HotStuff use threshold signatures rather than multi-signatures. Both threshold signatures and
multi-signatures have $O(1)$ pairing cost but multi-signatures require $O(n)$ group operations for adding 
public keys, which accounts for the higher latency (see Table 1).

\par \textbf{Replica Performance}. We find that Wendy's reliance on the Oz no-quorum proof allows it to minimize replica verification time without sacrificing optimistic responsiveness. Figure~\ref{fig:verification} measures 
verification latency as a function of number of participants. Both Fast-Hostuff and SBFT's latency grows linearly with $f$. 

Although in Fast-HotStuff the replica only needs to verify $O(1)$ signatures,
the verification of the aggregate signature requires $O(n)$ pairings and $O(n)$ group operations. SBFT has the
same pairing complexity and $O(1)$ group operation complexity; however, the cost of pairings dominate. SBFT has
$4x$ higher latency than Fast-HotStuff, however, since SBFT has to verify both QCs and votes so the constants
for the pairing cost are higher than Fast-HotStuff. Two-Chain HotStuff and Wendy have similar verification
performance until $f=33$, after which the $O(n \log{n})$ group operation complexity increases the latency about
$50x$ compared to Two-Chain HotStuff. Although, Two-Chain HotStuff has lower latency compared to Wendy, this is
at a cost of not being responsive, which leads to being slower in the terms of leader performance. Wendy still 
maintains a $50x$ latency reduction compared to Fast-HotStuff and $250x$ latency reduction compared to SBFT.
This is because of the $O(1)$ pairing complexity, which is the primary bottleneck of the replica performance.
So even though Wendy has higher group operation complexity, in practice it is much faster than Fast-HotStuff and
SBFT because of the $O(1)$ pairing complexity.


\subsection{Bandwidth}
In addition to performance, we also measure the bandwidth of each protocol's view change. We first fix the batch
size at $100$KB and then measure bandwidth as a function of $f$. For $f<100$, the bandwidth is dominated by the
$100$KB batch size, however, for $f>100$ the $O(n^2)$ authenticator add about a $100x$ increase in bandwidth. 
Since Fast-HotStuff uses multi-signatures rather than threshold signatures it has an additional factor of $n$
increase in bandwidth because each QC must maintain a bitmap of which public keys were used for signing. Wendy
and Two-Chain HotStuff have both $O(n)$ authenticator complexity, so for $f<3333$, they maintain nearly the same
bandwidth but for $f>3333$ the $O(n^2 \log{n})$ bit complexity adds about a $20\%$ increase in bandwidth. In
comparison to Fast-HotStuff and SBFT, Wendy saves about $77x$ and $15x$ of bandwidth. For our next experiment we
fix $f=333$ for a total of $1000$ replicas, and measure the bandwidth as a function of batch size. For batch sizes
less than $1$MB the bit and authenticator complexity dominates the bandwidth but past $1$MB the batch size is
the dominant factor of bandwidth and the additional increase in complexity is negligible. For smaller batch
sizes the authenticator complexity dominates bandwidth compared to bit complexity. The additional $n \log{n}$
increase in bit complexity from Wendy to Two-Chain HotStuff only results in a $1\%$ increase in bandwidth.

\subsection{Storage}
Finally, we measure the storage overhead of Wendy compared to the other protocols. The aggregate signature scheme
Wendy uses requires storing $O(n^2 \log{n})$ public keys and proofs of possession and $O(n \log{n})$ secret keys.
In contrast SBFT and Two-Chain HotStuff only require storing $O(1)$ public keys, $O(1)$ secret keys, and no 
proofs of possession. Fast-HotStuff uses multi-signatures so that requires storing $O(n)$ public keys and
proofs of possession but it only requires $O(1)$ secret keys. Thus from figure 9 the key storage overhead for
Wendy is about $145$MB for $f=10000$. Although SBFT and Two-Chain HotStuff have significantly less storage costs
compared to Wendy, these keys can all be easily kept in memory and storage costs are only a factor in a one-time 
bootstrap phase where replicas have to exchange public keys. In other words, the trade-off with additional
storage overhead is a small price to pay for a much more performant responsive protocol.















==> podc_2022/hotstuff.tex <==
\section{Motivating Example: HotStuff}
HotStuff is a leader speaks once protocol that has a \textit{strict} commit rule. 
This means that a
block is committed only when there have been three QCs in \textit{consecutive} views 
that reference a block.

This is necessary to preserve safety and liveness when there are view changes. Additionally,
modern BFT protocols like HotStuff rotate the leader every round in order to improve fairness,
and reduce the influence of any single replica. The combination of rotating the leader every
round with a strict commit rule is problematic with just \textit{crash} failures. We show
a liveness issue with HotStuff with just crash failures. This liveness issue then 
motivates
us to construct BFT protocols that have a \textit{relaxed} commit rule that allows a replica
to commit a block when there are QCs in non-consecutive views, thereby avoiding this liveness
issue.

\subsection{Leader Failures}
We first demonstrate a liveness issue in HotStuff with $n=4$ replicas, and a simple round-robin
leader rotation mechanism, which is the most commonly used.

\par \textbf{Crash Failure Example.} Suppose we have $n=4$ replicas, labeled $R1-R4$, with a round robin leader schedule
($R1$ is leader of view $1$, $R2$ leader of view $2$, etc.). Now suppose $R3$ crashed. $R1$ would propose a block $B$ in
view $1$, and $R2$ would certify it in view $2$. $R2$ would then propose a block $B'$ that extends $B$, and the replicas
would send their votes $R3$. Since $R3$ crashed, $R3$ would be unable to certify $B'$, and so a view change would be triggered.
$R4$ would collect the highest QCs from all replicas, and propose a block $B''$ that extends $B$ in view 4, since it is the highest
certified block. $R1$ would then certify $B''$ in view 5, however, $B$ cannot be committed because $B$ was certified in view $2$
and $B''$ was certified in view 5, which are not consecutive. So $R1$ would have to propose a block $B'''$ that extends
$B''$, and the replicas would send their votes to $R2$ in view $6$. $R2$ would then certify $B'''$ in view $7$ and commit
$B''$ (QCs in consecutive views), and thereby commit $B$. The issue is that since the commit rule requires two consecutive
QCs, liveness requires three consecutive honest leaders. Therefore, in this example it took $7$ views for $B$ to be committed
instead of $4$ if we just needed three honest leaders (not necessarily consecutive).

\par \textbf{Naive Fix.} To fix this issue, we could just relax the commit rule so that a block can be committed if it has
two QCs reference it (not necessary to have consecutive views). This change, however, is not safe, and  we show why with the following counterexample.
$R1$ proposes a block $B$ in view $1$, and the replicas send their votes to $R2$. $R2$ certifies $B$ in view $2$,
and then proposes a block that extends $B$. Because of an asynchronous network, a view change occurs, and the replicas send their highest QC to $R3$. $R3$ receives \textsc{NewView} messages from the $R1$, $R3$, and $R4$ replicas, and picks the highest
QC, which is for the genesis block. It proposes a block $B^*$ that extends the genesis block, the $R1,R3,R4$ quorum of replicas send 
their votes to $R4$, who certifies $B^*$, and proposes a block that extends $B^*$. Because of an asynchronous network, a view
change occurs before $R4$ broadcasts the proposed block. $R1$ then receives \textsc{NewView} messages from the $R1,R2,R3$ quorum
of replicas, of which the highest QC is for block $B$. $R1$ then proposes a block $B'$ that extends $B$, the $R1,R2,R3$ quorum of
replicas vote for $B'$, and send their votes to $R2$. $R2$ certifies $B'$

==> podc_2022/protocol.tex <==
\section{\sys{}}
\label{sec:protocol}

In this section, we present \sys, a new partially synchronous CLSO protocol that
satisfies Theorem \ref{thm:main}. \sys \xspace has optimal resilience ($f<n/3$), 
optimal latency of $2$ round-trips, and optimistic responsiveness. We conduct 
a formal analysis of its worst-case and expected throughput under failures in Section~\ref{sec:complexity}.

\sys{} provably achieves better latency and throughput than similar chained protocols \fs{that's a strong blanket statement... I assume you mean "under attack", i.e. the lat/tput in theory should not degrade (and thus its better)}. Our protocol addresses the liveness issue identified in Section~\ref{sec:background}: in the presence of omission faults, \sys{} simply requires a sequence 
of three (possibly non-consecutive) honest leaders. When commission faults
do occur, \sys{} reliably detects equivocation and immediately slashes the faulty replica, removing it from the
protocol. In contrast, prior work necessarily required three or four \textit{consecutive honest} leaders.

\sys's primary technical innovation lies in its \changebars{careful}{clever}\fs{avoid too self-congratulatory wordings} use of \textit{Equivocation} and \textit{No-QC} proofs to achieve gap-tolerance when possible. 
Equivocation proofs reliably indicate that a replica has misbehaved and should be slashed and removed from the system.
No-QC proofs, on the other hand, indicate that a QC \textit{could not have} formed for a specific block. The combination of these two proofs
is powerful. Knowledge that a QC \textit{definitely did not form} allows leaders to commit blocks that prior work could not have safely committed. When no such knowledge can be extracted, the replica  directly learns that the previous leader equivocated; an explicit \textit{equivocation proof}
allows for this node to be safely slashed. 

\changebars{Interestingly,}{} \sys{} leverages
\textsc{Vote-req} messages to implement equivocation proofs. \textsc{Vote-req} messages, in traditional BFT protocols, denote the first
round of messages sent by the leader, prior to any agreement having been reached. As it is easy for a malicious leader to equivocate at this stage,
\textsc{Vote-req} messages are traditionally excluded from the view change; they do not convey sufficient information. In contrast, they
are essential to \sys{},  which uses \textsc{Vote-req} messages to identify and blame faulty leaders, as well as prove that
a QC could not have formed for a specific block.
\fs{I'd reword this paragraph. To me, the message/insight is as follows: Existing protocols try to (because thats the natural intuition for the minimum bar for safety) recover any block that could have committed. The Vote-req information does not give me any extra information for this requirement -- thus there is no use in keeping it. Note, that Fast Path protocols instead MUST use it to maintain the safety guarantee, and thus will have it (However, they still don't use them for liveness-just for safety). We instead observe, that using them CAN be useful for the specific liveness scenario we are facing. We are interested in not only recovering blocks that could have committed, but also blocks by honest proposers that are in the commit process. Put differently: The Vote-Reqs are ignored because they dont affect safety. But they are important/useful for Liveness -- and that is the oversight existing work makes. The concrete thing we use vote-reqs for is to distinguish failure scenarios (i.e. omission/commission) --> which lets us identify honest (-appearing) proposers and maintain their progress. Note that, since we do use Vote-Reqs, we automatically support a Fast Path View Change too} 

We prove that \sys{} is both safe and live in Appendix~\ref{proofs}.

\subsection{Protocol Preliminaries}

We first introduce terminology and background.

\par \textbf{Views.} \sys{} progresses through a series of monotonically increasing \textit{views} with each view $v$ having a distinct leader $L_{v}$.
%We assume a simple round-robin leader rotation scheme, where the leader of view $v$, $L_{v}$, is determined by $v \mod n$.

\par \textbf{Fast View Change vs Slow View Change.} \sys{} replaces the leader on every view. As is standard in CLSO protocols, we distinguish between two types of view changes, the fast view change (FVC), and the slow view change (SVC). A FVC represents the steady state of the system: the leader of a new view certifies the block $B$ proposed in the previous view and proposes a new block $B'$ that has $B$ as its parent. The slow-view change,
in contrast, represents interrupted processing: sufficiently many honest participants indicated a belief that the past leader failed to respond. The new leader must aggregate sufficient information to reliably learn what happened in the previous view and continue the protocol.

\begin{figure*}
\fbox{\begin{minipage}{\linewidth}
\textbf{Quorum Certificate:}
\begin{itemize}
    \item $B$: block 
    \item $v$: view in which $B$ was proposed
    \item $\sigma$: set of $n-f$  \textsc{Vote-resp} messages in favor of $B$
\end{itemize}
\end{minipage}
}
\caption{\textbf{Quorum Certificate}}
\label{fig:qc}
\end{figure*}

\par \textbf{Quorum Certificates}. A QC consists of $n-f$ signatures on a block $B$ and has the following format $QC_B := (v, B, \sigma)$
(Figure~\ref{fig:qc}). $B$ is the block that the QC certifies and $v$ is the view of the QC. Note that $v$ is always equal to $B.v$
and thus refers to the view in which the block was initially proposed rather than the view in which the QC was formed. 
Finally, $\sigma$ is a signature or a set of signatures indicating $n-f$ replicas voted for $B$. A QC is valid if it is
well-formed and contains valid signatures. We say that a block $B$ has been \textit{certified} once a QC for $B$ has formed. 

\begin{figure*}
\fbox{\begin{minipage}{\linewidth}
\textbf{Block:}
\begin{itemize}
    \item $h$: the height of the block
    \item $H(B_{h-1})$: hash pointer to parent block
    \item $b_h$: batch of client transactions
    \item $v$: view in which block was proposed
    \item $QC$: QC attesting validity of parent block 
    \item $\sigma_l$: leader signature
\end{itemize}
\textbf{Additional state for a slow block:}
\begin{itemize}
    \item $S$: set of \textsc{NewView} messages
    \item $\pi$: optional equivocation proof
\end{itemize}
\end{minipage}
}
\caption{\textbf{Block Structure}}
\label{fig:blocks}
\end{figure*}

\begin{figure}
    \centering
    % Figure source: https://drive.google.com/file/d/1df2T-HQplE18dKQU1GWJG3JO8vtsajrL/view?usp=sharing
    \includegraphics[scale=0.9]{podc_2022/example_chain.pdf}
    \caption{Example chain of blocks in \sys{}. The shaded boxes represent slow blocks and the unshaded boxes represent fast blocks. Note that the $QC$ in a fast block is always for the parent block, however, this is not necessarily the case for slow blocks, as illustrated by block F.}
    \label{fig:example_chain}
\end{figure}

\par \textbf{Blocks and Block Format}. As is standard, \sys{} batches client requests into \textit{blocks}, with each block containing
a hash pointer to its parent block (or to null in the case of the \textit{genesis} block).
An example chain of blocks is given in Figure~\ref{fig:example_chain}. A block's position in the
chain is known as its height. There are two types of blocks (Figure~\ref{fig:blocks}): blocks formed in the steady-state FVC, \textit{fast blocks},
and blocks formed in the slow view change, \textit{slow blocks}. 
\begin{itemize}
    \item \textbf{Fast Blocks}. A fast block $B$ has the following structure: 
$B := (h,H(B_{h-1}), b_h, v, QC, \sigma_{\ell})$. $h$ denotes the height of the block in the chain. $H(B_{h-1})$ is a hash pointer to its parent block
(at height $h-1$), $b_h$ is a batch of client transactions, $v$ is the view in which
the block is proposed. $QC$ is a quorum certificate attesting to the validity of an ancestor of $B$. Finally,
$\sigma_{\ell}$ refers to the leader's signature of the block. 
\item \textbf{Slow Blocks}.  Slow blocks contain two additional fields $S$ and $\pi$.
$S$ refers to the set $S$ of \textsc{NewView} messages sent by replicas to the leader during a slow view change (more detail later).
$\pi$ denotes either an equivocation proof (defined more formally in~\S\ref{subsec:commit}) or $\bot$ if no equivocation
is detected.
\end{itemize}

A block is valid if 1) its parent block, if it exists, is valid 2) all included client transactions $b_h$
satisfy an application level validity predicate, and 3) all included signatures are valid.

\par \textbf{Block extension and conflicts}.  A block $B'$ extends a block $B$ ($B \longleftarrow B'$) if $B$ is an ancestor of $B'$: there 
must exist a path of parent blocks from $B'$ to $B$. Conversely, we say that $B'$ conflicts with $B$ if $\neg (B \longleftarrow B' \lor B' \longleftarrow B)$.
Informally, if $B'$ conflicts with $B$, these blocks are on separate forks of the chain and only one of them can commit. By convention, we say that blocks extend themselves ($B\longrightarrow B$).

\begin{figure*}
\fbox{\begin{minipage}{\linewidth}
\textbf{Replica Local State:}
\begin{itemize}
    \item $v_r$: current view number
    \item $QC_r$: the QC contained in $vr_r$
    \item $vr_r$: highest (by view) \textsc{Vote-req} message received 
   \item $vp_r$: highest (by view) \textsc{Vote-resp} message sent
\end{itemize}
\end{minipage}
}
\caption{\textbf{Replica Local State}}
\label{fig:localstate}
\end{figure*}

\par \textbf{Replica Local State.} Each replica $r$ maintains the following local state (Figure~\ref{fig:localstate}): $v_r$, the current view
number, $QC_r$, the QC received with the highest view, $vr_r$, the highest valid \textsc{Vote-req} message received, and
$vp_r$ the highest \textsc{Vote-resp} message sent. We discuss what \textsc{Vote-req} and \textsc{Vote-resp} messages are next.

\subsection{Fast View Change}

We first focus on the fast view change, which takes place in the absence of leader failures. Intuitively, the leader for view $v$ forms a valid QC for a block $b$ in view $v-1$. As the views are contiguous, no conflicting proposal could have been certified. The leader can then safely extend $b$ with a new proposal $b'$ and propose $b'$. FVC in \sys{} is identical to existing chained protocols, where each phase consists of two steps: 1) the leader proposes a block to all
replicas, with evidence that this block is on a valid chain 2) replicas certify the block and forward their vote to the leader of the next view.
We explain the protocol in more detail next and give pseudocode in Appendix~\ref{fast:vc}.

\par \textbf{Propose.} Let us assume that the leader for view $v$ (we write $L_v$) has already received $n-f$ signed replica votes of the form \msg{Vote-resp}{B_{v-1}} (we describe how these messages are generated below). $B_{v-1}$ is the proposal for view $v-1$. $L_v$ uses those replies to form a QC for $B_{v-1}$ attesting that a majority of honest participants have validated the block (we denote this QC as $QC_B$).  $L_v$ then proposes a new block $B_v$ that extends $B_{v-1}$. Extending $B_{v-1}$ is safe as $QC_B$ is necessarily the highest QC: 1) no QC could have formed between views $v-1$ and $v$ as these views are contiguous 2) a single QC can form per view as all QCs must overlap in at least one correct replica. 
%Block $B$ has as parent a hash to block $B.parent = B_{L_{v-1}}$, view $B.v=v$, and QC $B.QC = QC_B$. 
The leader signs this block and broadcasts a \msg{Vote-req}{B} message to all replicas. 

\protocol{\ul{Step 1: $L_v$ to all $R$} \\ Send \msg{Vote-req}{B_v} where $B=(h, H(B_{v-1}), b_h, v, QC_B, \sigma_L)$} 

%
%\par \textbf{Pre-Prepare.} \The steady state for view $v$ begins when $L_v$ forms a QC for a block proposed in the previous view, $QC_B$,
%by gathering $n-f$ signed \emsg{\msg{Pre-Prepare}{B}{$L_{v-1}$}}$_r$ messages, where $B.v=v-1$. This QC has the highest possible view (since it was for a block in the previous view). No conflicting QC could have formed in an intermediate view, it is therefore safe and live for the leader to extend this QC \fs{Again: I doesn't seem like the highest view extension rule was described anywhere so far}. The leader
%then proposes a new block $B'$ s.t. $B'.parent=B$, $B'.v=v$, and
%$B'.QC=QC_B$, by broadcasting a \msg{}{B'}$_{L_v}$ message to all replicas.

\par \textbf{Vote.} When a replica receives a valid \msg{Vote-req}{B}$_{L_v}$ message, 
it validates that it is in the correct view, that it has not already voted in this view, and that the proposal is valid. Specifically, the
replica checks that it is in the same view as the leader (that $B.v = v_r$), and that $B$'s QC attests
a block in the preceding view $v-1$ (that $B.QC.v = v_r-1$). The
replica then simply update its local state to reflect the received messages and votes to
support the block. Specifically, it updates $QC_r$ to $B.QC$ and highest received \textsc{Vote-req} message $vr_r=$ \msg{Vote-req}{B}$_{L_v}$. 
The replica then sends a signed \textsc{Vote-resp} message to the leader of view $v+1$, acknowledging its support for $B_v$
and stores the message locally (in $vp_r$).

\protocol{\ul{Step 2: $R$ to $L_{v+1}$} \\ Send \msg{Vote-resp}{B_v}$_{\sigma_R}$}

We highlight that, unlike all other CLSO protocols, replicas in \sys{} explicitly stores Vote-requests for a block $B$ \textit{before}
$B$ has achieved agreement. Replicas in Hotstuff for instance, only update their local state once a QC on block $B$ has already formed.
As we will see next, this small change is key to achieving gap-tolerance for omission faults.

\par \textbf{Steady State Commit.} 
When a replica sends a \msg{Vote-Resp}{B_v} message, it checks to
see whether it can commit any blocks from previous views. Specifically, it
fetches the past two certified blocks: $B_2=B_v.QC.B$ and $B_1=B_2.QC.B$, and their 
associated QCs: $QC_1$ and $QC_2$. If they are in consecutive views (which is the case in the steady state), that is 
$QC_2.v == QC_1.v+1$, then it is safe for the replica to commit $B_1$. Note that this
commit rule is the same as prior CLSO BFT protocols. The main novelty of \sys{} is the
commit rule for when QCs are not in consecutive views, which is how \sys{}
maintains safety while also satisfying \textit{Non-CHLC}. 

\subsection{Slow View Change}
%\fs{normalized Vote-req, Vote-resp captialization across section 5; also normalized sigma R to be capital (sometimes it was lowercase); TODO: make consistent with remaining sections and proofs.}

The fast view change in \sys{} is simple: as views are contiguous, the new leader is guaranteed to learn the latest certified block and can thus easily extend the chain. There is no such continuity in the slow view change, which requires
more care.  A slow view change is triggered when sufficiently many replicas fail to receive a new block proposal before a specific timeout value; replicas vote to move on to the next view and transfer necessary state to new leader. It is no longer possible for a leader to simply extend \changebars{the highest certified}{a} block, as conflicting blocks could have been proposed during views that did not complete. \sys{} makes careful use of the stored highest \textsc{Vote-req} message ($vr_r$) to address this challenge. \changebars{}{To achieve gap-tolerance in the presence of crash failures, \sys{}
ensures that no block that \textit{could have been certified} but for the crash/omission failure of a faulty node, will be reproposed.} We include pseudocode in Appendix~\ref{slow:vc}.

\par \textbf{New View.} Each replica in view $v-1$ sets a local timer after sending a \textsc{Vote-resp} message. If no new block is received before the timer expired, the node votes to start a new view. Specifically, it 
%increments its current view to $v_r = v$ (and will no longer process messages in lower views) and 
sends a signed \textsc{NewView} message to the leader of this new view $v$. \textsc{NewView} messages include
the replica's current view $v_r$ and the highest received QC ($QC_r$). Importantly, the message also includes the highest received \textsc{Vote-req} message ($vr_r$) as well as the highest stored response ($vp_r$).
As previously stated, sending \textsc{Vote-req} messages as part of the view change
is unique to \sys{}. 

\protocol{\ul{Step 1: $R$ to $L_v$} \\ Send \msg{NewView}{v,QC_r, vr_r, vp_r}$_{\sigma_R}$}


%Hotstuff, for instance, sends only \textit{precommitQCs} (that is, QCs for blocks that have already gone through the agreement phase of the protocol). Similarly, PBFT includes only its equivalent \textit{prepare certificates} ($2f+1$
%pre-prepare messages, which ensures that a single command could commit in this particular slot).

\par \textbf{Propose.} Once in the new view, the new leader, $L_v$ waits for $2\Delta$
time to collect \textsc{NewView} messages from all honest replicas. We will show shortly
why this is necessary for liveness. Like the FVC, $L_v$ must pick a block to extend for
its proposal; however, since there is not a QC for $v-1$, $L_v$ must carefully pick a
block to extend such that it maintains safety across views. To do so, $L_v$ finds the
$vr_r$ (\textsc{Vote-Req}) with the highest view among the set of \textsc{NewView}
messages it receives. There could, however, exist ties, so those are broken by the view
of the contained QC ($vr_r.B.QC.v$). And ties on the view of the QC can be broken 
arbitrarily. Once $L_v$ identifies a block $B$ that it must extend, for liveness it tries 
to form a QC with a higher view than $B.QC$ that $B$ extends. To do so it iterates
through the ancestors of $B$, stopping at $B.QC.B$, and checks to see whether there
exists $2f+1$ $vp_r$ in the set of \textsc{NewView} messages, for a more recent ancestor
block than $B.QC.B$. If so, $L_v$ forms a QC, $QC_{anc}$. $L_v$ then gathers a new batch
of client transactions, $b_h$, and proposes a new slow block $B'$ that extends $B$, 
contains
$QC_{anc}$ if it exists (otherwise $B.QC$), the new view $v$, the set of \textsc{NewView}
messages it received, and a signature on the block $B'$. It then multicasts a
\msg{Vote-Req}{B'} to all replicas.

\protocol{
\begin{enumerate}
    \item Wait $2\Delta$
    \item Find the \msg{Vote-Req}{B} message in the set $S$ of 
    \textsc{NewView} messages with the highest view (highest $B.v$), break ties on 
    the highest QC view ($B.QC.v$), break further ties arbitrarily.
    \item \begin{enumerate}
        \item Initialize $B^*=B$ and $QC_{anc}=B.QC$. 
        \item Loop until $B^*.v \leq B.QC.v$
        \item If there exists $2f+1$ $vp_r$ messages in $S$, where
        $B^* \longleftarrow vp_r.B$, then set $QC_{anc}$ to be the QC formed on $B^*$. 
        \item Set $B^*=B^*.parent$
    \end{enumerate}
    \item $B'=(H(B),b_h,v,QC_{anc},\sigma_{L_v},S)$, where $\sigma_{L_v}$ is a signature on $B'$
\end{enumerate}
\ul{Step 1: $L_v$ to $R$} \\
Send \msg{Vote-Req}{B'}$_{\sigma_{L_v}}$ to all replicas}


%The new leader, $L_v$, has two key responsibilities: 1) choosing the correct
%block to have its new proposal extend, and 2) certifying any blocks in the chain 
%that have $n-f$ votes. These two responsibilities are simple in the fast view change, as the new leader 
%receives $n-f$ votes for the block proposed in the previous view, which allows $L_v$ to certify it, and
%propose a new block that extends it. These responsibilities are more complicated in the slow view change since 
%previous views may not have finished entirely. Responsibility 1 is necessary to preserve safety, otherwise
%conflicting forks can be committed. Responsibility 2 is necessary to preserve liveness, otherwise a faulty
%leader can prevent blocks from being certified (and thus committed) indefinitely. We first describe the
%procedure and intuition for the safety responsibility (responsibility 1), and then discuss the same for the
%liveness responsibility (responsibility 2).

%\par \textbf{Preserving Safety.} To ensure safety, if a block was committed 
%in a prior view, the new leader, must extend it with its new proposal. Thus,
%the new leader thus must extend any block that \textit{could have been}
%committed. The rule for picking which block to extend is the following: 
%\begin{itemize}
%    \item Find the \msg{Vote-Req}{B} message in the set $S$ of 
%    \textsc{NewView} messages with the highest view (highest $B.v$)
%    \item Ties on $B.v$ are broken according to highest QC (highest $B.QC.v$)
%    \item Ties on $B.QC.v$ are broken arbitrarily
%\end{itemize}

\fs{I want to point out that voting with just the High-QC would be enough for safety. Using the high Vote-Req is ALSO safe, because it's strictly more information (it includes the High-QC as prefix -- like you show). But to me the "why" we pick vote-req is for liveness, not safety. Here you answer: "why is picking vote-req STILL safe"}
\neil{I see your point, and this is really applicable for the case where the 
highest vote-req contains the highest qc. In the case that the highest
vote-req doesn't contain the highest qc we know that both the highest qc
(because of the no commit proof) and the the highest vote-req (because of 
the guaranteed equivocation proof from the highest qc) could not have been 
committed. Nevertheless whether picking the highest vote-req 
(containing the highest qc) or 
highest qc; it's still about maintaining safety. The certification of past
blocks with vote-resp is the liveness part}

\par \textbf{Vote.} When a replica receives a valid \msg{Vote-req}{B'}$_{L_v}$ message, 
it validates that it is in the correct view, that it has not already voted in this view, and that the proposal is valid. Specifically, the
replica checks that it is in the same view as the leader (that $B'.v = v_r$), the
highest \textsc{Vote-Req} in $B'.S$ breaking ties by the QC view is the parent block of 
$B'$, the highest valid ancestor QC of $B$ is indeed $B'.QC$ (using the \textsc{Vote-Resp}
messages in $B'.S$). The
replica then simply update its local state to reflect the received messages and votes to
support the block. Specifically, it updates $QC_r$ to $B'.QC$ and highest received \textsc{Vote-req} message $vr_r=$ \msg{Vote-req}{B'}$_{L_v}$. 
The replica then sends a signed \textsc{Vote-resp} message to the leader of view $v+1$, acknowledging its support for $B'$ and stores the message locally (in $vp_r$).

\protocol{\ul{Step 2: $R$ to $L_{v+1}$} \\ Send \msg{Vote-resp}{B'}$_{\sigma_R}$}

\par \textbf{Commit.} Once a replica sends a \msg{Vote-resp}{B'} message, it checks
whether it can commit any blocks from previous views. Like the steady state commit, it
fetches the past two certified blocks: $B_2=B'.QC.B$ and $B_1=B_2.QC.B$ and their
associated QCs: $QC_2$ and $QC_1$. It then iterates through all of the slow ancestor 
blocks of $B_2$, stopping at $B_1$, checking to see whether any slow ancestor block
contains, in its set of \textsc{NewView} messages, a \msg{Vote-Req}{B}, which contains in 
its ancestry an equivocation proof for view $B_1.v$. This equivocation proof consists of
at least two \textsc{Vote-Req} messages for different blocks but with view $B_1.v$.
This equivocation proof constitutes evidence that the leader of $B_1.v$ was Byzantine,
and the existence of $QC_2$ ensures that $2f+1$ replicas have observed this equivocation
proof, which allows us to maintain safety.

\protocol{
\ul{Commit Rule}
\begin{enumerate}
    \item $B_2=B'.QC.B$, $B_1=B_2.QC.B$
    \item Initialize $B^*=B_2$
    \begin{enumerate}
        \item Loop until $B^*.v \leq B_1.v$
        \begin{enumerate}
            \item Iterate through every $vr_r.B$ in $B^*.S$
            \item Initialize $B_s=vr_r.B$
            \begin{enumerate}
                \item Loop until $B_s.v \leq B_1.v$
                \item If $B_s.S$ contains an equivocation proof for view $B_1.v$, ABORT, slash
                the leader of $B_1.v$
                \item $B_s = B_s.parent$
            \end{enumerate}
        \end{enumerate}
        \item $B^* = B^*.parent$
    \item If no equivocation detected then commit $B_1$
    \end{enumerate}
\end{enumerate}
}


\par \textbf{Why extend the highest \textsc{Vote-Req}?} By the commit rule, when a 
block, $B$ is committed, $n-f$ replicas must 
have updated their $vr_r$ to be \msg{Vote-Req}{B'}, and their $vp_r$ to 
\msg{Vote-Resp}{B'}, where $B'.QC$
certifies block $B$. By quorum intersection, the set $S$ of \textsc{NewView} 
messages received by $L_v$ must contain this \textsc{Vote-Req}. Therefore,
it is possible that an honest replica committed $B$ (the block certified
by $B'.QC$), so the new leader must pick the highest \textsc{Vote-Req}.





\par \textbf{Why break ties on the QC?} Suppose there exists two
\textsc{Vote-Req}s on blocks $B_1$ and $B_2$ respectively, where 
$B_1.v=B_2.v$ but $B_1.QC.v>B_2.QC.v$ (and these QCs conflict). 
In this case, even if $B_2$ is 
certified, it is not possible for $B_2.QC.B$ (the block certified by $B_2.QC$)
to be committed. The reason is that $B_1.QC$ exists with a higher view than
$B_2.QC.B$. In order for this QC to form it must be the case that there
was equivocation in view $B_2.QC.B.v$, otherwise $B_1.QC$ must have extended
$B_2.QC.B$. This equivocation will be seen by $n-f$ replicas
if $B_2$ is certified, so $B_2.QC.B$ will not be committed.

\par \textbf{Ensuring Liveness.} Note that certifying a block requires two leaders. 
The first leader sends the proposed block to all replicas, and the second leader collects
the votes and forms a QC. To ensure liveness, we need honest leaders to help certify
blocks proposed by honest leaders in prior views. 
Otherwise, if there is an honest leader followed by a Byzantine leader, then it
is possible that a block will never be certified (and therefore never committed). After choosing 
a block $B$ to extend, the new leader must iterate through all
of the ancestors of $B$ up until the latest certified block, $B.QC.B$, and try to certify any
blocks that have enough votes. To do so, the new leader waits a timeout to receive \textsc{NewView}
messages from all honest replicas. Then, it selects a block $B$ to have its new proposal extend.
The new leader sets $B^*=B$ and does the following:

\begin{enumerate}
    \item If there exists $n-f$ \textsc{Vote-Resp} messages for blocks that extend $B^*$, use them to
    certify $B^*$ (forming a quorum certificate, $QC^*$), and then stop.
    \item Otherwise, set $B^*=B.parent$, and repeat step 1. If $B^*=B.QC.B$, then stop.
\end{enumerate}

After completing this procedure, the new leader collects a batch of transactions and forms a block, $B'$,
where $B'.parent=B$, and $B'.QC=B.QC^*$ if $QC^*$ exists, OR $B'.QC=B.QC$ otherwise.


----------------------------------------OLD TEXT------------------------------------------------------------
\fs{where does this end?}
The new leader $L_v$ for view $v$ waits to receive $n-f$ \textsc{NewView} messages from replicas voting to enter view $v$.
We refer to this set as $S$. For safety, the leader must ensure that \changebars{its proposal in the new view extends all blocks that could have been committed.}{all blocks that could have been committed are included in the new view.}
This property is inherited from all prior CLSO protocols. To satisfy gap-tolerance in the presence of omission faults, the leader has additional
responsibilities: it must also certify all QCs that \textit{could have formed} in prior views that were led by faulty leaders, and who may have intentionally not completed the round.
%{\textit{would have formed} in prior views, but for a faulty leader preventing the view from completing}. 
For example, a leader in view $v_n$ will certify
%{would have to certify} 
a block $B$ proposed in view $v$ if all replicas in $v$ voted for $B$ but the leader in view $v+1$ fails to form and disseminate the corresponding QC.
%{failed to form a QC and disseminate it}.

\neil{I think it might be easier to reverse the order of the steps. 
We can start by saying that for safety you have to pick the correct block
to extend. And then the second step for liveness is that we have to certify 
any prior blocks that the correct block didn't extend}
To account for this, in a slow view change the leader proceeds in two steps. First, it certifies any block that had been implicitly agreed upon but whose certification process had been interrupted
by a faulty leader. To do so, it looks at the set of \textsc{Vote-req} messages received:
\begin{itemize}
    \item  if all $n-f$ \textsc{Vote-req} messages are for block $B_i$ in view $v_i$, the leader forms a new $QC_i = (B_i, v_i, \sigma_S)$ where $\sigma_s$
    denotes the set of corresponding \textsc{Vote-resp} messages. 
    %\fs{why is it using req messages here? Using Resp messages feels more intuitive: I.e. Resps are typically combined into QCs.} \fs{If you want to just use Req and cut Resp that seems fine too (I know Heidi had asked about this) -- I cannot discern why the else case below uses Resp though in that case.} 
    \item  otherwise, the leader identifies the greatest (by view) common ancestor of the $n-f$ blocks. If such a block $B_{anc}$ exists (and is not the genesis block), the leader forms a new $QC_{anc} = (B_{anc}, v_{anc}, \sigma_S)$ where $\sigma_s$
    denotes the set of \textsc{Vote-resp} messages.
\end{itemize}

Next, the leader must determine which block to extend. 

\changebars{In prior CLSO protocols, the leader extended the highest
certified block from the $n-f$ \textsc{NewView} messages it received. This
was to preserve safety, since a committed block is guaranteed to have its
corresponding QC appear at least once in the $n-f$ \textsc{NewView} messages
it received (by quorum intersection). In \sys{}, however, the 
\textsc{NewView} messages contain the highest \textsc{Vote-Req} from each
replica, $vr_r$, which gives the leader more information to determine
whether a block could have committed. We break down all the possible cases
in the slow view change, and show what \sys{} does to preserve safety.
}{
The highest QC in the $n-f$ \textsc{NewView} messages (we call it $QC_{high}$) certifies a block that may have committed (any committed block's QC 
%\fs{is this implicitly referencing the "PrepareQC" or the "CommitQC"? I'd say the prior since I assume you intend to convey that "at least one replica in the quorum will appear to be locked", but the wording is a bit ambiguous}
will appear
at least once in $n-f$ messages). It is thus necessary for any subsequent proposal to extend $QC_{high}$. Unlike prior work however, the leader must also consider the new implicit
QCs: $QC_{i}$ and $QC_{anc}$.
%\changebars{or}{and}\fs{since only 1 can exist? you said "otherwise" above} $QC_{anc}$.  
Specifically, it selects as its $QC_{choice}$ the QC with the highest view whose associated block extends $QC_{high}.B$. In other words $QC_{choice} = max (QC_{i}, QC_{anc}, QC_{high})$. Effectively,
%\fs{Effectively? I'm not sure whats the intuition here, see comment below}, 
the leader
upgrades its choice to one of the new implicit QCs if and only if this QC a more recent QC on the same branch as $QC_{high}$. 
%\fs{Can you say something more about this? I.e.: If Qi or Qanc did not extend Qhigh, then "clearly" (add intuition for why) it could not have actually committed, and hence its ok to ignore them? }
}

\changebars{The main considerations for the slow view change is the 
\textsc{Vote-Req}(s) with the highest view (we denote as $highVotes$), 
and the QC with the highest view (we denote $highQC$). The rule is to
always extend the \textsc{Vote-Req} with the highest view, and break ties by
the highest QC. We give the intuition for why this is safe by considering
each possible case in the view change.}{}

\begin{enumerate}
    \item No ties; highest \textsc{Vote-Req} extends highest QC
    \item No ties; highest \textsc{Vote-Req} does not extend highest QC
    \item Ties; tied \textsc{Vote-Req}s have different QCs
    \item Ties; tied \textsc{Vote-Req}s have same QCs
\end{enumerate}

\changebars{The safety intuition is that if a replica commits a block $B$,
then there must exist $n-f$ replicas which updated their $vr_r$ to be a 
\textsc{Vote-Req} that contains a QC for $B$. This means that in the view
change there will always exist at least one of these \textsc{Vote-Req}s,
and so the leader must extend this \textsc{Vote-Req} to maintain safety.
Note that even if there exists a lower \textsc{Vote-Req} with a higher QC,
we do not extend it since if it were committed there would have existed a
\textsc{Vote-Req} in the higher view.
}{}

Unfortunately, extending the latest QC only is not sufficient to achieve
gap-tolerance in the presence of omission faults. Some of the associated blocks
%\fs{associated with what? do you mean "proposed extensions of the branch QCchoice?} 
could have been received and acknowledged by $n-f$ replicas if the leader had not failed, and thus could have been implicitly certified. To preserve gap-tolerance, \sys{} must extend any such block. We distinguish between three cases:
%\neil{Add that there can be multiple \textsc{Vote-req} that have the highest view. In this case they are ranked first by the QC they contain but if they have the same QC then one is picked arbitrarily as highVote, and an equivocation proof is formed by the conflicting \textsc{Vote-req}}
\begin{itemize}
    \item The \textsc{Vote-req}
    %\fs{is stuff missing in the bracket?} 
    with the highest view (we write $highVote$) extends $QC_{choice}.B$
    (we write $QC_{choice}.B \longleftarrow highVote.B$). The leader directly extends $highVote$ in this case.
    \item $highVote.B$ does not extend $QC_{choice}.B$. The leader checks whether there exists $n-f$ \textsc{Vote-req} messages that do not contain $QC_{choice}$; if no such quorum exists %\fs{double negation with previous sentence is a bit hard to read-- is it even correct? Don't you mean "if such a quorum exists"? }
    , $QC_{choice}.B$ could not have committed. It is also safe for the leader to extend $highVote.B$.
    \item Otherwise, the leader sets $highVote$ to be the highest \textsc{Vote-req} that
contains %\fs{just contains --i.e. direct child --, or extends?}
$QC_{choice}$, since $QC_{choice}$ could have committed.
\end{itemize}
If multiple vote messages exist with matching views but non-matching blocks, the new leader has proof that the previous leader (of view $v-1$) equivocated.
The leader collects these conflicting votes and creates
an equivocation proof $\pi$ against the leader for that view, ensuring that all replicas will slash this malicious node. 

Finally, the leader collects this information and creates a new slow
block $B_v$ containing as parent $highVote.B$, a set of new transactions $b_H$, the set of \textsc{NewView} messages $S$ and any equivocation proofs. The replica broadcasts
this new block as part of a \textsc{Vote-req} message.
%\heidi{what happend to HighVote.B?} \natacha{Fixed. Neil, can you please double check?}

\protocol{\ul{Step 1: $L$ to all R} \\ Send \msg{Vote-req}{B}$_{\sigma_{L_v}}$ with $B=(h,H(highVote.B), b_h, v, QC_{choice}, S,  \pi, \sigma_{L_v})$}
%\fs{We never actually seem to use/need the height h at all. Does it make (hypothetical) implementation easier, or is it included mainly to make it easier to talk about "no two conflicts" at the same height? (next section)}

\par \textbf{Replica Logic.} When a replica $r$ receives a \msg{Vote-req}{B} message with
slow block $B$, it performs two steps. First, it checks whether a replica was slashed
($B.\pi \neq \bot$ and $\pi$ is valid). $r$ will ignore all subsequent messages
received from a faulty replica. Second, it validates the 
vote message, confirming that the leader did in fact extend the correct
block. If the check passes, the replica votes to support $B$ and updates
its local state as in the fast view change protocol. 

\protocol{\ul{Step 2: $R$ to $L_{v+1}$} \\ Send \msg{Vote-resp}{B}$_{\sigma_R}$}

%\par \textbf{How does this ensure liveness?} Consider a replica $r$ which has a QC for 
%block
%$B_{k}$ in view $v$. Since a QC consists of $2f+1$ signed \textsc{Pre-Prepare} messages, at
%least $n-f$ replicas must have a $highPP.v \geq v$. This quorum of $n-f$ replicas intersects
%any quorum of \textsc{NewView} messages in at least $n-2f$ replicas, of which at least $1$ is honest.
%Thus, in the view change, the leader is guaranteed to see at least $1$ honest replica with a \textsc{Pre-Prepare} for $B_{k}$. 

Prior CLSO protocols %\natacha{Add a list of CLSO protocols here}, 
such as HotStuff (\S\ref{sec:background}) explicitly discard all proposed blocks for which a replica has not received confirmation that the block has been certified. Block certification enforces agreement: once
a replica receives a QC for a block $B$, it can be certain that no conflicting block will commit at that height and in that view. Past protocols assume that only certified blocks should be included in the view-change.  HotStuff, for instance, only
includes \textit{precommit QCs} in the view-change and discards prepared messages. This approach is not limited to CLSO protocols.
PBFT includes only its equivalent \textit{prepare certificates} ($n-f$) in the view-change and discards
single \textsc{PRE-PREPARE} messages. %\fs{Punchline? In sys we observe instead that this information is crucial to preserve liveness?}

%, have a view change protocol that has the leader collect at least $n-f$ messages 
%containing each replica's highest QC (by view). 
%The leader picks the highest QC received. Recall that each QC is associated with a particular block $b$ and a set of replicas who voted in favor of that block. The leader then \textit{extends} this QC by proposing a new block with $b$ as its direct parent.
%These view change protocols only consider QCs, and not blocks that replicas have voted for but
%have not been certified (a QC has not formed for the block). The main observation of our
%protocol is that these votes provide extra information that allow replicas to detect
%equivocation or not miss the latest block that \textit{could have been certified}. Thus,
%instead of a replica only tracking the highest QC it received, it also tracks the highest
%block (by view) it have voted for. Additionally, in the view change protocol instead of the
%leader proposing a new block whose parent is the block the highest QC refers to, the leader
%proposes a new block whose parent is the highest voted block (by view), who has an ancestor
%(a path following parent blocks) to the highest QC block. To see the advantage of this
%approach, suppose a QC formed in some view $v$. If a view change occurs in $v+1$ it is possible
%that this QC does not appear in the $n-f$ messages containing the highest QC each replica
%has received (since this QC may not have reached enough replicas), that the leader of $v+1$ collects. However, it must be the case that $n-f$ replicas have their latest vote for this 
%block in view $v$, which intersects the $n-f$ messages the leader of $v+1$ receives in at
%least 1 honest replica. Thus it is guaranteed that the leader of $v+1$ sees at least 1 vote.
%Similarly, by the same quorum intersection argument if there does not exist a vote for the
%block in the view change then a QC for the block could not have formed. In our protocol
%we call the message in which the leader proposes a block as \textsc{Pre-Prepare}, and the
%message which indicates a replica voted for a block as a \textsc{Pre-Prepare} message signed
%by the replica who voted. \fs{I don't see the difference here.. haha}
%%


\subsection{Commit Rule and Slashing}\label{subsec:commit}

% What point is it safe to commit a block, no explicit messages, phases like in non-chained protocols

Unlike traditional BFT protocols, CLSO systems do not have an explicit commit phase. They must instead determine when it is safe to mark a block as committed 
using a \textit{commit rule}. Committing a block implicitly also commits all of its ancestors. 

Intuitively,  a block $B$ is safe to commit and execute if all replicas agree, across views, that this block is the only block at height $h$ that could commit. 
Achieving this property necessarily requires at least two phases (and thus two QCs). The first QC certifies $B$ and achieves agreement across replicas: no other QC can form for a conflicting block $B'$ in the same view $v$. The next QC achieves persistence across views: subsequent leaders in views $v'>v$ will extend $B$. 

Traditionally, these QCs must form in consecutive views. The commit rule in \sys{}, however, is more refined: it is safe to commit a block with non-consecutive QCs \textit{as long} as one can prove that no conflicting
QCs formed in intermediate views. \sys{} once again 
%\fs{referring to what? -- *this* is what they are for} 
leverages \textsc{Vote-req} messages to generate No-QC proofs that precisely prove that no QC formed in a view. \sys{} additionally uses these messages to reliably detect any leader that successfully caused a conflicting QC to form, and slashes this replica. Together, these properties allow \sys{} to achieve gap-tolerance.

% Commit rule:
% Need two QCs to commit, first QC ensures agreement, second QC ensures all subsequent view chances will see first QC and therefore extend it. Note that when you commit a block, you also
% implicity commit all of its ancestors. 
% Traditionally, these QCs
% need to be consecutive. Our commit rule is more refined. We are saying that, even if they are not consecutive, it is *still* possible to commit as long as we are able to
% create a No-QC proof for any view in between.

Specifically, when replica $r$ receives a new block $B_r$ 
%\fs{any reason the underscore is r, as in replica r? It's not meant to indicate this block was proposed by r is it?} 
with associated QC $QC_r$, it checks which blocks in the chain can now be committed and executed. Recall that two QCs are necessary to commit a block; the next block that can potentially be committed (we write $B_{commit}$) is then the block certified by the QC that $QC_r$ extends. For instance, consider what happens when a replica receives block G in Figure~\ref{fig:example_chain}. If $QC_r=QC_F$, $G$'s associated QC $QC_F$ certifies block $F$, and $F$'s associated QC $QC_{D}$ certifies block $D$, the
first committable block. Note that these blocks
are not necessarily direct parents of each other, as \sys{} allows for leaders to extend blocks in \textsc{Vote-req} messages directly. 
$r$ can safely commit $B_{commit}$ if there does not exist a QC that formed in a view between $QC_{commit}$ and $QC_{r}$. We
consider two scenarios: contiguous QCs and non-contiguous QCs. 

\begin{itemize}
\item \textbf{Contiguous QCs.} Two QCs are contiguous if $QC_r.v = QC_{commit}.v + 1$. It is trivially safe to commit $B_{commit}$  as there does not exist an intermediate view in which a conflicting QC could have formed.  
\item \textbf{Non-Contiguous QCs.} If the QCs are not contiguous, one must confirm that there does not exist a conflicting block $B_{conflict}$
with a view greater than $v_{commit}$ that has been certified. In other words, 
there must not exist a QC of the from $QC_{conflict} = (v, B_{conflict}, \sigma)$ where $v>QC_{commit}.v$ and $v < QC_r.v$. If such QC exist, it is not safe to commit %\fs{which block?}
$B_{commit}$.
%{: $r$ could mark $B_{commit}$ as committed in this view.} \fs{flow before read really weird to me}. 
In a later view, however, a different leader could observe both $QC_{commit}$ and $QC_{conflict}$ as part of a later view-change and choose to extend $B_{conflict}$ as $QC_{conflict}$ has a higher view. This new leader would in effect be overwriting $B_{commit}$'s commit decision, violating
safety. To convince itself that no such $QC_{conflict}$ exists, $r$ leverages \textsc{Vote-req} requests to generate an explicit \textit{No-QC proof}. We know that, by
quorum intersection, if a block $B_{conflict}$ has been certified, all subsequent leaders will observe at least one \textsc{Vote-req} message for $B_{conflict}$
(certifying a block requires $n-f$ votes; at least one honest node's vote is guaranteed to be included in the next view). $r$ thus checks every block
on the chain 
%\fs{can you clarify in text what it means to "check a block"? I assume it means to "check the n-f proof messages that came along with the Vote-Req block proposal" I.e. QC for fast VC, and set S for slow VC (or is it only these?); in either case the replica possibly needs to also acquire intermediary QC's (or VC quorums) for blocks that are on the branch but were not locally received? } 
between $B_r$ (included) and $B_{commit}$ to determine whether such a conflicting \textsc{Vote-req} exists. Fast-blocks occur in contiguous views and thus do not need to be checked (they do not store \textsc{Vote-req} messages).  For slow blocks,  $r$ checks that there does not exist a \textsc{Vote-req}
message that is for a conflicting block $B*$ in the same or higher view; a block $B*$ conflicts with $B_{commit}$ if  $B_{commit} \nleftarrow B*$ 
%\fs{you mean B* instead of Bconflict?}.  
The absence of such \textsc{Vote-req} message constitutes a No-QC proof; $r$ can safely commit $B_{commit}$. 
%\fs{Minor: This whole paragraph sounds like r is generating the proof, when so far I always read it as "the leader submits either a No-QC proof or an Equiv proof", which the replica will eventually "consume". Probably not important, but tripped me up for a second because as soon as I read "r generates.." I got confused whether its the leader or any replica (the latter of which the paragraph said before).}
\end{itemize}

\par \textbf{Slashing} The use of No-QC proofs guarantees gap-tolerance in the presence of omission faults, but may not succeed when malicious leaders explicitly equivocate.
%{says nothing about cases in which malicious leaders explicitly equivocated}. 
Fortunately, the commit logic described above can be repurposed to simultaneously reliably detect commission failures.
%{leveraged to also reliably detect commission faults}. 
If a malicious leader
successfully causes subsequent leaders to create a QC for a conflicting block $B_{conflict}$, the same quorum intersection argument guarantees that at least one honest leader replica
will observe conflicting \textsc{Vote-req} messages in $B_{commit}$'s
view. To understand this claim, let $B_{conflict}$ be the earliest certified block that does not extend $B_{commit}$ and let $QC_{conflict}$ be the associated QC. As $QC_{commit}.v < QC_{conflict}.v$ 
%\fs{why? the previous sentence does not imply this by itself. It could be an ancestor? Are trying to imply that since Bcommit is committed (by assumption) the commit rule guaranteed that there was no conflict in smaller view? Is Bconflict meant to be conflicting (it doesnt say yet)}
, it must be the case that the leader in $QC_{conflict}.v$ observed at least one vote for a block that extends $B_{commit}$ (by quorum intersection).  The only way in which a leader can legitimately propose $B_{conflict}$ is if it extends a \textsc{Vote-req} message for a conflicting block $B_{req}$, such that $B_{req}.v \geq B_{commit}.v$. Let $vreq$ be the first such \textsc{Vote-req} that does not extend $B_{commit}$.
Since $B_{commit}$ was certified, by quorum intersection $vreq$ must include 
%\fs{you mean the quorums on the branch of vreq include it? Or directly in Breq.S?} 
a \textsc{Vote-req}
for $B_{commit}$, and $vreq$ is the earliest \textsc{Vote-req} that does not extend $B_{commit}$ with view $\geq B_{commit}.v$, $vreq$ must have the same view as $B_{commit}.v$. 
%\fs{The whole previous sentence confuses me} 
However, $vreq$ conflicts with $B_{commit}$, forming an equivocation proof.

%\fs{Minor: I've noticed that here you implicitly use "conflict" in terms of branches that are not prefix of one another, whereas above conflicting was just for 2 blocks at the same height. Maybe harmonize it to define somewhere that two blocks conflict, if their branches conflict? (from which it follows that two blocks at same height h conflict)}

These conflicting \textsc{Vote-req} messages form an equivocation proof,
which replicas will use as evidence to exclude
the faulty replica from the protocol.  After $f$ equivocation attempts, all faulty replicas will be removed from the system,
thus guaranteeing that the protocol will always successfully generate No-QC proofs and commit $B_{commit}$. 

% \heidi{add a sentence somewhere on state transfer}
% QC_B.v = QC_r.v + 1, easy! Safe to commit. Why, because no intermediate QC for a conflicting block could have formed
% If not in contiguous views, want to check that there does exist a block B-conflict that has been certified (there exists a QC of the form QC = (v, B, sigma)).  and has a higher view than B. 
% This matters because for safety, in a future view,  this conflicting QC could overwrite that committed decision, because it's in a higher view. 
% So how do we prove this? 
% B conflict is not certified if, for every view between B_r.v and B.v, there does not exist a Vote-req for b_conflict. THe reason is that you need 2f+1 to certificate, which means your'e guaranteed
% at least once Vote-req. So keeping Vote-req around is again what allows us to generate this noQC proof, and achieve gap tolerance in the absence of equivocation. 
% Next, we start from B_r and check every block in the past until B to determine whether there is a No-QC proof. B is guaranteed to be an ancestor of B_r. B_r extends the QC for B, and so we know that it either directly extends B
% or extends a Vote-req that extends B. Let's call the current block we're considering B*. Fast blocks don't have Vote-reqs but they are trivially safe / slow blocks, we need to look at the set of Vote-reqs, and if none of them
% are for a conflicting block B* conflict (note it does not have to be the same b conflict),then we're doomed and commit rule is not satisfied.  
% If your'e not able to commit, there must exist at least one replica (the leader in the Vote-req message view) that equicated, we know for sure this replica is Byz, and so we can slash it and use conflicting Vote-reqs as an equivocation proof, much
%%like in the slow view change. Which means that this can happen for at most f blocks after which we can always apply the contiguious or non contiguous rules, achieving gap tolerance. 
%\par \textbf{Commit.} When a replica $r$ updates its $QC_r$, it checks whether a block $B$ can 
%be committed. For the commit rule, $r$ looks at the QCs, $QC_r$ and $QC_B = QC_r.B.QC$. \fs{the right equation side is kind of hard to parse. Is this just the locally stored QC for B? }
%The intuition for the commit rule is that it is only safe to commit $B$ if there does not
%exist a higher QC for a conflicting block. To do so, $r$ must check every ancestor block of
%$QC_r.B$ until $B$ to see whether there exists any corresponding \textsc{Pre-Prepare} message 
%for the
%conflicting block. If there does not exist such \textsc{Pre-Prepare} then it is proof that
%no conflicting higher QC could have formed. \fs{below here is quite difficult to read/follow; might benefit from expanding a tad}
%More formally, $r$ has to check whether it is possible that a $QC'$ formed s.t.
%$B \nleftarrow QC'.B$ and $QC'.v > QC_B.v$. By a quorum intersection argument, if there exists
%a \emsg{\msg{Pre-Prepare}{B'}$_{L_{B'.v}}$}$_r$ s.t. $B'.v>B.v$ and $B \nleftarrow B'$ then
%it is possible $B'$ was certified.
%Therefore $r$ checks all of the ancestor blocks of $QC_r.B$ to see whether there are any
%\emsg{\msg{Pre-Prepare}{B'}$_{L_{B'.v}}$}$_r$ s.t. $B'.v>B.v$ and $B \nleftarrow B'$.
%If not, then it is proof that a higher conflicting $QC'$ does not exist, so it is safe to
%commit $B$. In the case that $QC_r$ and $QC_B$ are in consecutive views, the commit rule
%is trivially satisfied. 
%
%\par \textbf{How does this preserve safety?} 
%In the view change the leader collects at least $n-f$ \textsc{NewView} messages containing the highest (by view) QC the replica has seen. The leader then extends this QC by proposing a new block that has a direct parent pointer to the
%QC's block. Note that even though the leader extends the highest QC, this is not necessarily the globally highest QC. Since the leader collects \textsc{NewView} messages from only $n-f$ replicas, there could exist a higher QC that only one
%of the other $f$ replicas have seen. Such a QC is often referred to as a hidden QC. Even though it is safe to extend the highest QC from $n-f$ replicas with a consecutive commit rule, it no longer necessarily becomes safe with a relaxed
%commit rule. \fs{perhaps actually highlight the old and new commit rule side by side when you state it the first time} This is because a hidden QC can overwrite a committed decision. Suppose during a view change for view $v$ the highest received QC from $n-f$ replicas was in view $v'$ but there exists a hidden QC in view $v''>v'$. If the QC in view
%$v'$ is committed, the hidden QC in view $v''$ can overwrite this committed decision and cause different honest replicas to commit different blocks resulting in a safety violation. This is not an issue with a consecutive commit rule since consecutive
%QCs guarantee that there does not exist a conflicting hidden QC that could overwrite a committed decision. \fs{Does Wendy avoid this hidden QC too? If so this should be clear in this para. If not, then there should be a forward reference to when it will be addressed}
%
%\par \textbf{Slash.} If $B$ cannot be committed because there exists a
%\emsg{\msg{Pre-Prepare}{B'}$_{L_{B'.v}}$}$_r$ s.t. $B'.v>B.v$ and $B \nleftarrow B'$,
%then it implies that there must exist some view, $v'$, where there were multiple highest
%\textsc{Pre-Prepare} messages. This implies that a faulty replica equivocated.
%A replica can then find use the conflicting \textsc{Pre-Prepare} messages in the
%same view as proof of equivocation. This equivocation proof can be used to slash and exclude
%the faulty replica.
%
%\par \textbf{How is this an equivocation proof?} Because a malicious leader can equivocate it is possible
%that there are multiple \textsc{Pre-Prepare} messages containing different blocks for the same view. If at any point an honest replica observes multiple \textsc{Pre-Prepare} messages
%in the same view for different blocks then this is proof of equivocation for the leader who
%sent those \textsc{Pre-Prepare} messages. An honest replia can use this proof to slash the
%faulty replica. This proof can be added to the chain to slash the faulty replica and replace
%or exclude this replica in the future. 
%
%\par \textbf{Why is it unsafe commit?} Equivocation, however, presents the following challenge: suppose there are
%multiple highest conflicting \textsc{Pre-Prepare} messages that extend the highest QC. There
%is not enough information to know which (if any) of those \textsc{Pre-Prepare} messages
%led to the formation of a potentially higher QC that was not seen in the $n-f$ messages the 
%leader received in the view change.
%If ties are broken arbitrarily then it is possible to 
%miss a QC that formed, making it unsafe to commit in non-consecutive views. This QC may have
%been missed because in the view change the leader collects the highest QCs from $n-f$ replicas,
%which means it is possible that a QC formed but not received by enough replicas to guarantee
%its inclusion in the view change.
%\fs{Clarify this section: You are describing Wendy's limitation correct? I.e. that Wendy can preserve liveness without consecutive views only when there is no equivocation. If there is equivocation, Wendy too must degenerate to the normal consecutive view requirement; With the positive caveat that it keeps Slashing the equivocating replicas, until there technically cannot be anymore equiv.}
%
\subsection{Communication Complexity.} 
Protocol logic is independent of the specific signature scheme chosen; protocol complexity, however,
is tightly coupled with this choice.
In the view change protocol, the leader sends a block
containing $O(n)$ \textsc{Vote-req} messages and $O(n)$ QCs to $O(n)$ replicas. Each
QC consists of $O(n)$ words (each word consisting of a digital signature), thus resulting
in $O(n^{2})$ words. Each \textsc{Vote-req} consists of $O(1)$ words, and thus a block
contains $O(n^{2})$ words in total, resulting in a total communication complexity of
of $O(n^{3})$ words. If threshold signatures are used, each QC can be reduced $O(1)$ words,
since a threshold signature is a single signature indicating a threshold of $k=n-f$ replicas
signed a message. This reduces the complexity to $O(n^{2})$ words. 
When instantiated with SNARKs, \sys{} achieves $O(n)$ complexity. %\natacha{Ittai, confirm?}
%Instead of a block
%containing the QCs and \textsc{Vote-req} messages themselves, the leader could attach a
%SNARK, which proves that the block contains $n-f$ valid \textsc{Vote-req} and QCs. This
%SNARK is $O(1)$ words, resulting in $O(n)$ word complexity if SNARKs are used.

%\begin{figure*}
%\fbox{\begin{minipage}{\linewidth}
%%Let $v$ be the current view number. Each replica $r$
%%maintains the following local state: $v$, the current view number, $QC_r$, the highest QC
%%replica $r$ has received, and $pp_r$, the highest \textsc{Pre-Prepare} message $r$ has received
%%signed by $r$.
%\textbf{Local State:}
%\begin{itemize}
%    \item $v$: the current view number
%    \item $QC_r$: the highest QC replica $r$ has received
%    \item $pp_r$: the highest \textsc{Vote-req} message $r$ has received
%\end{itemize}
%For the steady state protocol, a replica $r$ 
%runs the following steps in iterations for every view:
%\begin{enumerate}
%    \item \textbf{Pre-Prepare.} Upon receiving $n-f$ valid matching 
%    \emsg{\msg{Pre-Prepare}{B}$_{L_{v-1}}$}$_r$, if $L_v$
%    then form a quorum certificate $QC_B$ for B using this set of \textsc{Pre-Prepare} messages, gather a batch of client transactions, $b'$, and create a new block 
%    $B' := (H(B), b', v, QC_B)$ and broadcast \msg{Pre-Prepare}{B'}$_{L_v}$ to all replicas.
%    \item \textbf{Vote.} Upon receiving a valid \msg{Pre-Prepare}{B'}$_{L_v}$ message in view $v$, a 
%    replica $r$ checks that $B'.QC.v=v-1$, if so sets $QC_r=B'.QC$ and $pp_r=$
%    \emsg{\msg{Pre-Prepare}{B'}}$_r$, and finally sends $pp_r$ to $L_{v+1}$
%    \item \textbf{Commit.} See the commit rule figure ~\ref{fig:wendy-commit}.
%\end{enumerate}
%\end{minipage}
%}
%\caption{\textbf{Steady State Protocol}}
%\label{fig:wendy-ss}
%\end{figure*}
%
%\begin{figure*}
%\fbox{\begin{minipage}{\linewidth}
%Let $v-1$ be the current view number and replica $L$ be the leader of view $v$. Each replica
%$r$
%maintains the following local state: $v_r$, the current view number, $QC_r$, the highest QC
%replica $r$ has received, and $pp_r$, the highest \textsc{Pre-Prepare} message $r$ has received.
%A replica $r$ 
%runs the following steps in iterations for every view:
%\begin{enumerate}
%    \item \textbf{NewView.} Upon view timeout expiring in $v-1$, 
%    send \msg{NewView}{v,QC_r,pp_r}$_r$ to $L_v$
%    \item \textbf{Pre-Prepare.} After view synchronization wait $2\Delta$, and upon receiving a set $S$ of $n-f$ valid \msg{NewView}{v,QC_r,pp_r} messages, if $L_v$ then:
%    \subitem form any QCs for ancestor blocks from set of $n-f$ \textsc{Pre-Prepare} messages
%    \subitem gather all $n-f$ $QC_r$, and set $highQC$ to be the QC with the highest view
%    \subitem gather all $n-f$ $pp_r$, and set $highPP$ to be the $pp_r$ with the highest view that extends $highQC.B$ (if ties break arbitrarily, and set $\pi$ to be set of conflicting
%    \textsc{Pre-Prepare} messages for the same view, otherwise $\pi=\bot$)
%    \subitem gather a batch of client transactions $b'$ and create a block that extends
%    $highPP.B$, $B':=(H(highPP.B), b', v, S, \pi)$, and broadcast 
%    \msg{Pre-Prepare}{B'}$_{L_v}$ to all replicas
%    \item \textbf{Vote.} Upon receiving a valid \msg{Pre-Prepare}{B'}$_{L_v}$, a replica $r$ does the following:
%    \subitem checks that $B.S$ contains $n-f$ valid QCs and \textsc{Pre-Prepare}
%    messages
%    \subitem computes $highQC$ and $highPP$ to be the QC and \textsc{Pre-Prepare} respectively with the highest view in $S$
%    \subitem checks that $B'$ extends $highPP.B$, and $highPP.B$ extends $highQC.B$
%    \subitem sets $QC_r$ to be $highQC$ if $highQC.v>QC_r.v$, and signs and sets $pp_r$ to be
%    \emsg{\msg{Pre-Prepare}{B'}$_{L_v}$}$_r$
%    \subitem sends $pp_r$ to the leader of view $v+1$, if all checks pass.
%    \item \textbf{Commit.} See the commit rule figure ~\ref{fig:wendy-commit}.
%\end{enumerate}
%\end{minipage}
%}
%\caption{\textbf{View Change Protocol}}
%\label{fig:wendy-vc}
%\end{figure*}
%
%\begin{figure*}
%\fbox{\begin{minipage}{\linewidth}
%\begin{enumerate}
%    \item \textbf{Commit.} Upon updating $QC_r$ to a newer QC check the commit rule:
%    Let $QC_B=QC_r.B.QC$ and $B=QC_r.B$.
%    \subitem Let $B^*=QC_r.B$, and check that $B^*$ does not contain any \textsc{Pre-Prepare} 
%    messages for a block that conflicts with $QC_B.B$. If so set $B^*=B^*.parent$ and repeat
%    until $B^*=QC_B.B$, and if no conflicting \textsc{Pre-Prepare} messages were
%    found commit $QC_B.B$. If $QC_r$ and $QC_B$ are in consecutive views this is trivially
%    satisfied.
%    \item \textbf{Slash.} Upon scanning blocks for the commit rule if there is an equivocation
%    proof $\pi \neq \bot$ or if there exists multiple \textsc{Pre-Prepare} messages in the same
%    view $v$, for different blocks then detect equivocation and slash the faulty replica.
%\end{enumerate}
%\end{minipage}
%}
%\caption{\textbf{Commit Rule}}
%\label{fig:wendy-commit}
%\end{figure*}
%
%


==> podc_2022/protocol_proofs.tex <==
\section{Proofs}\label{proofs}

\subsection{Safety}

We first prove safety, defined below.

\begin{definition}
(Safety). Honest replicas do not commit conflicting blocks.
\end{definition}

\begin{definition}
(Block Extension). A block $B'$ extends block $B$ (denoted as $B \longleftarrow B'$), if $B$
is an ancestor for $B'$: there must exist a path of parent blocks from $B'$ to $B$.
\end{definition}

\begin{definition}
(QC Extension). A block $B'$ extends certificate $QC_{B}$ (denoted as $QC_{B} \longleftarrow B'$), if $B'.QC$ certifies a block, $B^*$ such that $B \longleftarrow B^*$
\end{definition}


\begin{definition}
(Conflicting blocks). Two blocks, $B$ and $B'$ conflict, if 
$\neg (B \longleftarrow B' \lor B' \longleftarrow B)$ ($B$ and $B'$ do not extend each other).
\end{definition}


%\begin{definition}
%(Global commit). We say a block $B$ is globally committed if $f+1$ honest replicas
%have a $vr_r$ (\textsc{Vote-REQ} message) for block $B'$, such that $B'.QC$ certifies $B$, and
%on the path of blocks from $B$ to $B'$ there does not exist a \msg{Vote-REQ}{B''}, 
%where $B''.v>B.v$, and $B''$ does not extend $B$.
%\end{definition}

%\begin{lemma}\label{lem0}
%If an honest replica commits $B$ due to the commit rule being satisfied, then $B$ is globally
%committed.
%\end{lemma}

%\begin{proof}
%By the commit rule, if an honest replica commits $B$ then there must exist $QC_B$, $B'$, and
%$QC_{B'}$ such that $B'$ contains $QC_B$, and on the path of blocks from $B$ to $B'$ there does
%not exist a \msg{Vote-REQ}{B''}, where $B''.v>B.v$, and $B''$ does not extend $B$. The existence
%of $QC_{B'}$ implies that $f+1$ honest replicas did have a $vr_r$ for $B'$.
%\end{proof}

%\begin{lemma}
%If a block $B$ is globally committed then any block $B^*.v>B'.v$ must contain a $highVote$ of
%view at least $B'.v$ containing a QC with view at least $B.v$.
%\end{lemma}

%\begin{proof}
%By the global commit definition, $f+1$ honest replicas set their $vr_r$ to \msg{Vote-REQ}{B'}
%and $QC_r$ to $B'.QC = QC_B$ (the QC that certifies $B$). Since $highVote$ is never decreased,
%a \textsc{NewView} message sent by any of the above $f+1$ honest replicas must be for view at
%least $B'.v$ containing a QC for a view at least $B.v$. By quorum intersection any set of $n-f$
%\textsc{NewView} messages in $B^*.S$ must contain a $vr_r$ message from at least one of these
%honest replicas.
%\end{proof}

\begin{lemma}\label{lem1}
If a quorum certificate, $QC_B$ forms for block $B$, then no other quorum 
certificate, $QC_{B'}$ can form for block $B'\neq B$ with $B'.v=B.v$.
\end{lemma}

\begin{proof}
Suppose for the sake of contradiction that $QC_{B'}$ did form for block $B'$. This means that a
quorum, $Q'$, containing $n-f$ replicas voted for $B'$. Denote the quorum of $n-f$ replicas 
that voted for $B$ as $Q$. $Q' \cap Q$ in at least $1$ honest replica. This honest replica
voted for both $B$ and $B'$ even though they both have the same view, a contradiction.
\end{proof}

\begin{lemma}\label{safety:lem3}
If an honest replica $r$ commits a block $B$, then let $QC_B$ be the QC that certifies $B$ and let $QC_{B*}$ be
the QC that certifies block $B*$ with $B*.v>B.v$ and $B \longleftarrow B*$, which causes $r$ to 
commit $B$, then no conflicting QC can form in a view $v'$ $B.v < v' < B*.v$
\end{lemma}

\begin{proof}
Assume for the sake of contradiction that a QC,
$QC_{B'}$, formed for a conflicting block $B'$. This implies that a quorum
$Q'$, s.t. $|Q'|=n-f$ voted for $B'$ in view $B'.v$. In view $v'$, every replica in $Q'$ must 
have updated its local $vr_r$ to be a valid \textsc{Vote-REQ} message containing $B'$. 
Let $B_1$ be the ancestor block of $B*$ with the lowest view such that $B_1.v > B'.v$. 
$B_1$ must conflict with $B'$, since $B*$ extends $B$. Since $B_1$ is the earliest block
that conflicts with $B'$ it must be the case that $B_1$ is a slow block containing a 
quorum of $n-f$ 
\textsc{Vote-REQ} messages since it does not extend $B'$. This quorum must intersect
$Q'$ in at least one honest replica, implying that $B^*.S$ must contain a 
\textsc{Vote-REQ} for a block that extends $B'$. Replica $r$, however, committed $B$ which means 
that for all blocks in the path from $B$ to $B*$, there must not be a \textsc{Vote-REQ} 
for a conflicting block, a contradiction since there must exist a \textsc{Vote-REQ} that extends
$B'$ in $B_1$.
\end{proof}


\begin{theorem}\label{safety:one}
If an honest replica $r$ commits a block $B$, then it must vote for a \textsc{Vote-REQ} containing
a $QC_{B^*}$ for $B^*$, where $B 
\longleftarrow B^*$ and $B^*.v > B.v$, which contains
a $QC_B$ for $B$. For any \msg{Vote-REQ}{B'} such that $B'.v > B^*.v$, that an honest replica
votes for, it must be the case that $QC_B \longleftarrow B'$.
\end{theorem}

\begin{proof}
We prove the theorem by induction.
\par \textbf{Base Case: $v'=B^*.v+1$}. Since there exists a $QC_{B^*}$, it must be the case that
at least $f+1$ honest replicas have a $vr_r$ for $B^*$. By quorum intersection at least one of
these $vr_r$ must be present in the view change for $v'$. This $vr_r$ will have the highest view
unless the leader of $B^*$ equivocates and there are multiple \textsc{Vote-REQ} messages with
view $B^*.v$. Since there cannot exist a $QC'$ for a block that conflicts with $B$ and a higher
view than $B$ by Lemma~\ref{safety:lem3}, it must be the case that if the leader does not extend $B^*$ it will extend a
\textsc{Vote-REQ} that contains a block that extends $QC_B$.

\par \textbf{Step.} We assume the theorem holds for all $v'-1 > B^*.v$, and now we
consider view $v'$. Suppose for the sake of contradiction there exists a \msg{Vote-REQ}{B'}
with view $B'.v=v'$ that does not extend $QC_B$. 
$B'$ must be a slow block since by strong induction any certified
block in $v'-1$ must have extended $B$. Thus $B'.S$ must contain $n-f$ \textsc{Vote-REQ} messages.
From the base case there must be at least $f+1$ $vr_r$ \textsc{Vote-REQ} messages that contain
$QC_B$. In order for $f+1$ honest replicas to vote for \msg{Vote-REQ}{B'}, $B'.S$,
must contain a \msg{Vote-REQ}{B_1}, where $B_1.v > B.v$ and $B^*$ conflicts with $B$. By the
base case and induction assumption $B_1.v \leq B^*.v$, and by quorum intersection $B_1$ must contain at least one
\textsc{Vote-REQ} that has view at least $B^*.v$ that contains a block that extends $QC_B$. However, $B'$ extended a conflicting \textsc{Vote-REQ} for $B_1$ with a lower view and lower QC, a
contradiction.
\end{proof}


%\begin{theorem}\label{safety:one}
%If an honest replica $r$ commits a block $B$, then for every block $B'$ that is certified s.t.
%$B'.v > B.v$, $B \longleftarrow B'$.
%\end{theorem}

%\begin{proof}
%We prove the theorem by cases. Let $QC_B$ be the QC that certifies $B$ and let $QC_{B*}$ be
%the QC that certifies block $B*$ with $B*.v>B.v$ and $B \longleftarrow B*$, which causes $r$ to 
%commit $B$.

%\par \textbf{Case $B'.v < B*.v$}. Assume for the sake of contradiction that a QC,
%$QC_{B'}$, formed for a conflicting block $B'$. This implies that a quorum
%$Q'$, s.t. $|Q'|=n-f$ voted for $B'$ in view $B'.v$. In view $v'$, every replica in $Q'$ must 
%have updated its local $vr_r$ to be a valid \textsc{Vote-REQ} message containing $B'$. 
%Let $B_1$ be the ancestor block of $B*$ with the lowest view such that $B_1.v > B'.v$. 
%$B_1$ must conflict with $B'$, since $B*$ extends $B$. Since $B_1$ is the earliest block
%that conflicts with $B'$ it must be the case that $B_1$ is a slow block containing a 
%quorum of $n-f$ 
%\textsc{Vote-REQ} messages since it does not extend $B'$. This quorum must intersect
%$Q'$ in at least one honest replica, implying that $B^*.S$ must contain a 
%\textsc{Vote-REQ} for a block that extends $B'$. Replica $r$, however, committed $B$ which means 
%that for all blocks in the path from $B$ to $B*$, there must not be a \textsc{Vote-REQ} 
%for a conflicting block, a contradiction since there must exist a \textsc{Vote-REQ} that extends
%$B'$ in $B_1$.

%\par \textbf{Case $v' \geq B*.v$}. We prove the theorem by induction.
%\par \textbf{Base Case: $v'=B*.v$}. By lemma ~\ref{lem1} there can be at most one QC
%in a given view, and since there is already a $QC_{B*}$ for a $B*$ that extends $B$, there
%cannot be a conflicting certified block with view $B*.v$.

%\par \textbf{Step.} We assume the theorem holds for all $v'-1\geq B*.v$, and now we
%consider view $v'$. Suppose for the sake of contradiction there exists a certified block $B'$
%with view $B'.v=v'$ that does not extend $B$. 
%This implies that at least $f+1$ honest replicas voted for a 
%\msg{Vote-REQ}{B'} message. $B'$ must be a slow block since by strong induction any certified
%block in $v'-1$ must have extended $B$. Thus $B'.S$ must contain $n-f$ \textsc{Vote-REQ} messages.
%From the base case there must be at least $f+1$ $vr_r$ \textsc{Vote-REQ} messages that contain
%$QC_B$ that extend $B$. In order for $f+1$ honest replicas to vote for \msg{Vote-REQ}{B'}, $B'.S$,
%must contain a \msg{Vote-REQ}{B_1}, where $B_1.v > B.v$ and $B*$ conflicts with $B$. Since
%$B$ was committed, by case $B.v < B'.v < B*.v$, and by strong induction $B_1.v < B.v$, a
%contradiction.

%The formation of $QC_{B*}$ implies that $f+1$ honest replicas have a
%$vr_r$ containing $QC_B$ for a block that extends $B$, and furthermore, from the first case and
%induction hypothesis it must be the case that any QC for a block that conflicts with $B$ must
%have a view $< v$. $f+1$ honest replicas intersect the view change quorum in $v'$ in at
%least one honest replica, which implies that there will be a $QC_r$ and $pp_r$ that extends
%$B$ in the view change. Since any conflicting QC must be for a lower view, the leader of $v'$
%must propose a block that extends $B$ for at least $f+1$ honest replicas to vote in $v'$. 
%Otherwise, no honest replica will vote a \textsc{Pre-Prepare} that does not extend $B$, so
%any QC that forms in $v'$ must be for a block that extends $B$.
%\end{proof}

\begin{theorem}
For any two committed blocks $B$ and $B'$ by an honest replica then either $B \longleftarrow B'$ 
or $B' \longleftarrow B$.
\end{theorem}

\begin{proof}
By Theorem~\ref{safety:one}, if an honest replica commits $B$ ($B'$) then every valid 
\textsc{Vote-REQ} that an honest replica votes for in a future view must contain a QC that extends
$QC_B$. Since a QC requires at least $f+1$ honest votes, it must be the case that every later
certified block must extend $B$ ($B'$). Since only certified blocks can be committed, any pair of
certified blocks cannot conflict.
\end{proof}

\subsection{Liveness}

Liveness depends on a critical component called the pacemaker or view synchronization
mechanism. There are many pacemakers such as Cogsworth~\cite{naor2020cogsworth} 
and FastSync~\cite{bravo2020making}. Any of these pacemakers can be used with this protocol. We assume the pacemaker 
satisfies the following theorem.

\begin{theorem}\label{live:thm1}
Let $v$ be a view with an honest leader after GST. Within time bound of $T_f$ 
from when the first honest
replica enters $v$, all honest replicas also enter $v$ and receive a proposed block $B$.
\end{theorem}

We now prove optimistic bounds for when there is no equivocation by faulty replicas.

\begin{lemma}\label{live:lem1}
Assuming no malicious leader equivocates, after GST and view synchronization, 
if an honest leader multicasts \msg{Vote-REQ}{B} then 
then any valid \msg{Vote-REQ}{B'}, s.t. $B.v \leq B'.v \leq v$, must extend $B$.
\end{lemma}

\begin{proof}
We prove the lemma by induction.

\par \textbf{Base Case: $B'.v=B.v$}. By theorem ~\ref{live:thm1}, it must be the case that 
all honest replicas will enter $B.v$ and receive \msg{Vote-REQ}{B}$_{L_{B.v}}$ within time 
bound $T_f$. Since the $L_{B.v}$ is honest, it will not equivocate and only send
\msg{Vote-REQ}{B}$_{L_{B.v}}$ to all replicas. It will be the only valid \emsg{Vote-REQ} message
in view $B.v$ and all honest replicas will 
update their $vr_r$ and send
a \msg{Vote-RESP}{B} message. The lemma is satisfied since $B \longleftarrow B$.

\par \textbf{Step}. We assume the lemma holds $\forall v'$ s.t. $B.v<B'.v<v$ and now consider 
$B'.v=v$. Suppose for the sake of contradiction there does exist a valid \msg{Vote-REQ}{B'} s.t.
$B'.v=v$ and $B'$ does not extend $B$. By strong induction all valid \textsc{Vote-REQ} messages
in $v-1$ must extend $B$, therefore $B'$ must be a slow block. Since $B'$ does not extend $B$,
$B'.S$ must contain a \msg{Vote-REQ}{B^*} message, where $B^*$ conflicts with $B$. By quorum 
intersection, $B'.S$ must contain a \textsc{Vote-REQ} message with view at
least $B.v$ that extends $B$. By strong induction \msg{Vote-REQ}{B^*} must have the property that
$B^*.v < B.v$. Since \msg{Vote-REQ}{B^*} has a lower view, the only way \msg{Vote-REQ}{B'} is valid
is if $B^*.QC.v > B.QC.v$ and $B.S$ contains at least one \textsc{Vote-REQ} containing $B^*.QC$ 
out of $n-f$ messages. 
Since $L_v$ is honest, $B.S$ must contain at least $n-f$ \textsc{Vote-REQ} messages that
do not contain $B^*.QC$, as otherwise $B$ would have extended $B^*.QC.B$ and not $B.QC.B$, a
contradiction.
\end{proof}



%\begin{lemma}\label{live:lem1}
%Assuming no malicious leader equivocates, after GST and view synchronization, 
%if an honest leader broadcasts $B$ then $\forall v'$ s.t. $B.v \leq v' \leq v$, where $v$ is
%the next view after $B.v$ with an honest leader, all honest replicas will have a $vr_r$ and
%corresponding $vp_r$ s.t. $B \longleftarrow vr_r.B$.
%\end{lemma}

%\begin{proof}
%We prove the lemma by induction.

%\par \textbf{Base Case: $v'=B.v$}. By theorem ~\ref{live:thm1}, it must be the case that 
%all honest replicas will enter $B.v$ and receive \msg{Vote-REQ}{B}$_{L_{B.v}}$ within time 
%bound $T_f$. Since the $L_{B.v}$ is honest, 
%\msg{Vote-REQ}{B}$_{L_{B.v}}$ will be valid and all honest replicas update their $vr_r$ and send
%a \msg{Vote-RESP}{B} message. The lemma is satisfied since $B \longleftarrow B$.

%\par \textbf{Step}. We assume the lemma holds $\forall v'$ s.t. $B.v<v'<v$ and now consider 
%$v'=v$.
%From the induction hypothesis in view $v-1$ all honest replicas must have a $vr_r$ and $vp_r$ s.t.
%$B \longleftarrow vr_r.B$. There are two cases: either the leader of $v$ receives $n-f$
%\msg{Vote-RESP}{B'}$_{L_{B'.v}}$ ($vp_r$)
%messages, where $B \longleftarrow B'$ and $B'.v=v-1$ (triggers the fast view change) or the 
%leader of $v$ receives $n-f$ \textsc{NewView} messages (triggers the slow view change).

%\par \textbf{Fast View Change.} With $n-f$ matching \msg{Vote-RESP}{B'}$_{L_{B'.v}}$ messages, 
%$L_{v}$ can form a QC for $B'$.
%This QC has view $v-1$, which is the previous view (at the time of view $v$). 
%$L_{v}$ can propose a new fast block $B''$ containing a QC for $B'$ with 
%$B''.parent=H(B')$. Since $L_v$ is honest and it is after GST, all honest replicas will receive
%a \msg{Vote-REQ}{B''} message and update their $vr_r$ and $vp_r$. This satisfies the lemma since
%$B \longleftarrow B' \longleftarrow B''$.

%\par \textbf{Slow View Change.}
%The set $S$ of $n-f$ \textsc{NewView} messages received by $L_v$
%must intersect all honest replicas ($n-f$ in total) in at least 
%$n-2f$ ($f+1$) honest replicas. 
%These honest replicas must
%have sent a \textsc{NewView} message containing a $vr_r$ s.t. $B \longleftarrow vr_r.B$.
%A Byzantine replica, however, can have a $vr'$ s.t. $B \nleftarrow vr'.B$, and $vr'.B$ has
%the highest view. $L_v$ will only extend $vr'$ if $vr'.QC.v$ is higher than any other
%$vr_r.QC.v$ from $S$. From the base case, all honest replicas must have a $vr'.QC.v$ that is
%at least $B.QC.v$. From strong induction all $vr_r$ from views $B.v$ to $v-1$ from honest replicas
%must for a block that extends $B$. Therefore it is impossible that a byzantine replica has a QC
%for $B'$ s.t. $B \nleftarrow B'$ and $B.v < B'.v < v$, since this requires at least $f+1$ $vp_r$
%messages from honest replicas, and thus $vr'.B.QC.v < B.v$. If $B$ is a fast block, then it is
%the case that $B.QC.v=B.v-1$, and so by Lemma ~\ref{lem1}, $vr'.B.QC.v<B.QC.v$, so $L_v$ will
%not extend $vr'.B$. If $B$ is a slow block, then it is possible that $vr'.B.QC.v>B.QC.v$. This,
%however, implies that $B.S$ contains $n-f$ valid \emsg{Vote-REQ} messages that do not include
%$vr'.B.QC$, since otherwise $B.QC=vr'.B.QC$. By quorum intersection $vr'.B.S$ must
%contain at least $f+1$ \emsg{Vote-REQ} messages containing $B.S$ (by extension). This implies 
%$vr'$ will be considered invalid since it extended a QC that has $f+1$ $n-f$ \emsg{Vote-REQ}
%messages that do not include it.

%From the base case every $pp_r.v \geq B.v$. Suppose for the
%sake of contradiction that $L_{v-1}$ sent a \msg{Pre-Prepare}{B^*}$_{L_{v-1}}$, where 
%$B^*.v=v-1$ and $B \nleftarrow B^*$. An honest replica will only accept this 
%\textsc{Pre-Prepare} if it extends the highest \textsc{Pre-Prepare} in $B^*.S$. Since
%there are at least $n-2f$ $pp_r \in B^*.S$ s.t. $B \longleftarrow pp_r.B$ and $pp_r.v \geq B.v$, this implies there exists a valid \textsc{Pre-Prepare}, $pp^*$, s.t. $B \nleftarrow pp^*.B$ and
%$pp^*.B.v > B.v$. If an honest replica had a $pp_r=pp^*$, this would contradict the base
%case and induction hypothesis.
%Since $L_{B.v}$ is honest there could not
%have been any equivocation in view $B.v$, and therefore it is impossible for a $pp^*$ s.t.
%$pp^*.B \geq B.v$ and $B \nleftarrow pp^*.B$ to exist in $B^*.S$, a contradiction.
%Thus, $L_{v-1}$ must multicast a \msg{Pre-Prepare}{B'}$_{L_{v-1}}$ where $B \longleftarrow B'$, so in $v-1$ all honest replicas can only update their $pp_r$ so that $pp_r.B = B'$, and since
%$B \longleftarrow B'$, the lemma is satisfied.
%\end{proof}

%\begin{lemma}\label{live:lem2}
%Assuming no malicious leader equivocates, after GST and view synchronization, 
%if an honest leader broadcasts $B$ then in view $v$, which is
%the next view after $B.v$ with an honest leader, all honest replicas will have a $QC_r$ s.t.
%$B \longleftarrow QC_r.B$.
%\end{lemma}

%\begin{proof}
%From theorem ~\ref{live:thm1}, after GST and view synchronization, once an honest replica $r$ enters view $v$ all honest replicas ($n-f$ in total) will enter $v$ and receive a proposed 
%block $B$ from the leader of $v$
%within $T_f$. From lemma ~\ref{live:lem1} for every view between $v$ and $v'-1$ all honest
%replicas will have a $pp_r$ s.t. $B \longleftarrow pp_r.B$. We again separate by cases on 
%whether the steady state or view change is triggered.

%\par \textbf{Steady State.} In the steady state the leader of $v'$ will receive $n-f$
%\emsg{\msg{Pre-Prepare}{B'}$_{L_{B'.v}}$}$_r$ messages, where $B'.v=v'-1$ and 
%$B \longleftarrow B'$. $L_{v'}$ will be
%able to form a QC for $B'$, and broadcast a \textsc{Pre-Prepare} for a new block $B''$, with
%$B''.parent=H(B')$. After view synchronization, within $2\Delta$ all honest replicas will 
%receive this \textsc{Pre-Prepare}, update its $QC_r$ to be for $B'$ since it has the highest 
%possible view (while in view $v'$) of $v'-1$, and $pp_r$, thus satisfying the lemma. 

%Upon updating its $QC_r$, an honest replica will check all of the
%ancestors of $B'$ to $B$ and check that there are no conflicting \textsc{Pre-Prepare}
%messages contained in a block with a view greater than $B.v$. If there is a conflicting
%\textsc{Pre-Prepare} with a greater view than $B.v$ then there must have been equivocation,
%since in $v$, $n-f$ honest are guaranteed to have a $pp_r$ for $B$. Since we assume no
%equivocation from views $v$ to $v'$, it must be the case there is no conflicting
%\textsc{Pre-Prepare}, and so it is safe to commit.

%\par \textbf{View Change.} After view synchronization, $L_{v'}$ will wait $2\Delta$ since
%$L_{v'-1}$ failed to make progress. This guarantees that $L_{v'}$ will receive a set $S$
%of $n-f$ \textsc{NewView} messages from honest replicas. 
%From lemma ~\ref{live:lem1} it is guaranteed that all
%honest replicas will have a $pp_r$ s.t. $B \longleftarrow pp_r.B$, and so 
%$S$ will contain 
%$n-f$ $pp_r$ messages s.t. $B \longleftarrow pp_r.B$. 
%$L_{v'}$ will form any QCs for any common ancestor blocks that are not certified, and thus will be able to form a
%QC for $B$ (if not already certified) and other blocks that extend $B$ that have $n-f$ signed \textsc{Pre-Prepare}
%messages. Since all honest replicas have a $pp_r$ with $B \longleftarrow pp_r.B$ from the
%base case and induction hypothesis, it must be the case that the highest QC is for a block
%$B'$ s.t. $B \longleftarrow B'$. Thus, $L_{v'}$ will pick the highest \textsc{Pre-Prepare},
%which must extend the highest QC, which must be for a block that extends $B$, to extend. It
%will propose a block $B'$, and after $2\Delta$ all honest replicas will receive a 
%\textsc{Pre-Prepare} for $B'$, and update its $QC_r$ and $pp_r$, thus satisfying the lemma.
%\end{proof}

We now prove the main theorem result of our paper (copied from the intro).

\begin{theorem}\label{live:mainthm}
After GST and view synchronization, if views $v<v'<v''$ have honest leaders, and 
block $B$ is proposed in view $v$,
then either block $B$ will be committed in view $v''$ or a previously undetected faulty replica
will be publicly detected and slashed (and excluded from any future participation).
\end{theorem}

\begin{proof}
From theorem ~\ref{live:thm1}, after GST and view synchronization, once an honest replica $r$ 
enters view $v$ all honest replicas ($n-f$ in total) will enter $v$ and receive a proposed 
block $B$ from the leader of $v$ within $T_f$, and send a \textsc{Vote-RESP} message within
$T_f+\Delta$.
From Lemma~\ref{live:lem1}, any \textsc{Vote-REQ} message between view $v$ and $v'$ must extend
$B$. If there is a fast view change in $v'$, then the leader of $v'$ will receive $n-f$ 
\textsc{Vote-RESP} messages that extend $B$, since by Lemma~\ref{live:lem1} any \textsc{Vote-REQ}
message in view $v'-1$ must extend $B$. If there is a slow view change in $v'$, then the leader
of $v'$ be guaranteed to receive \textsc{Vote-RESP} messages from all
honest replicas after $2\Delta$. Since the leader of $v$ was honest, all honest replicas will
have a $vp_r$ \textsc{Vote-RESP} message that extends $B$. Since there are at least $n-f$
\textsc{Vote-RESP} messages that extend $B$, the leader of $v'$ will be able to certify $B$. It
will then propose a block $B'$ that extends $B$, since the highest \textsc{Vote-REQ} message it
receives extends $B$. By a similar argument, the leader of $v''$
will be able to certify $B'$. By Lemma~\ref{live:lem1} any valid \textsc{Vote-REQ} message between
views $v$ and $v''$ must be for a block that extends $B$. Since there does not exist a conflicting
\textsc{Vote-REQ} message between views $v$ and $v'$, the commit rule is satisfied, and $B$ is
committed.


In the worst case when there is equivocation, there may exist a \textsc{Vote-REQ} message between
views $v$ and $v'$ that does not extend $B$, and thus $B$ cannot be committed. In this case, since
there is a record of the \textsc{Vote-REQ} messages, a malicious leader can be detected and
slashed if there exists conflicting \textsc{Vote-REQ} messages in the same view. Liveness
of the protocol falls back to requiring two consecutive honest leaders and a third honest leader
in a later view. With our equivocation detection mechanism and slashing,
faulty replicas will be severely punished for equivocation, so this fallback will occur
rarely. 

%From lemma ~\ref{live:lem1} for every view between $v$ and $v'-1$ all honest
%replicas will have a $pp_r$ s.t. $B \longleftarrow pp_r.B$. From lemma ~\ref{live:lem2} in
%$v'$ all honest replicas will have a $QC_r$ for block $B^*$ s.t. $B \longleftarrow B^*$.
%We now apply lemma ~\ref{live:lem1} again for views $v'$ through $v''-1$, and lemma
%~\ref{live:lem2} for view $v''$. This means that in view $v''$ all honest replicas have a
%$QC_r$ for block $B^{**}$ s.t. $B \longleftarrow B^* \longleftarrow B^{**}$. This triggers
%checking the commit rule. An honest replica $r$ will be able to commit $B^*$ and therefore
%$B$ (since committing a block commits all of its ancestors), if there does not exist a
%\msg{Pre-Prepare}{B'}$_{L_{B'}}$ s.t. $B'.v > B^*.v$ and $B^* \nleftarrow B'$. By 
%lemma ~\ref{live:lem1} from views $v$ through $v''$, all honest replicas will have a $pp_r$ 
%s.t. $B \longleftarrow pp_r.B$. Thus, the only way a conflicting \textsc{Pre-Prepare} forms
%in a view $v'>B.v$ is if a malicious leader equivocates. However, since all the honest
%accept a \textsc{Pre-Prepare} that extends $B$, $r$ can form an equivocation proof, $\pi$,
%by attaching the conflicting \textsc{Pre-Prepare} messages in the same view. Otherwise,
%since there are no conflicting \textsc{Pre-Prepare} messages in between it is safe to commit.

%If there is a conflicting
%\textsc{Pre-Prepare} with a greater view than $B.v$ then there must have been equivocation,
%since in $v$, $n-f$ honest are guaranteed to have a $pp_r$ for $B$. Since we assume no
%equivocation from views $v$ to $v'$, it must be the case there is no conflicting
%\textsc{Pre-Prepare}, and so it is safe to commit.
\end{proof}


We now bounds when there are commission faults (equivocation by faulty replicas).

\begin{theorem}
Let $v$ be some view after GST. Every honest replica eventually commits some block $B$ in
view $v'>v$.
\end{theorem}

\begin{proof}
Since we assume a round-robin leader rotation scheme, and the number of byzantine replicas is
bounded by $f$, by the pigeonhole principle we can find some view $v'$ such that
$v'$ and $v'+1$ have honest leaders. From theorem ~\ref{live:thm1} all honest 
replicas will enter
$v'$ and receive a proposal from the leader of $v'$ within $T_f$. 
Since the leader of $v'$ is honest. it will propose a block that is accepted by $n-f$ honest replicas, and they will send
their votes to the leader of $v'+1$ who is also honest after $T_f + \Delta$. The leader of $v'+1$ will form a QC, and propose
a block that extends it. After $T_f + 2\Delta$, $n-f$ replicas will update their $vr_r$ and $vp_r$
to reflect that they voted for it and send their votes to the leader of the next view.
Now consider $v''$, which is the next view after $v'+1$, which has an honest leader.
If $v''=v'+2$, the leader of $v''$ will receive $n-f$ votes within $T_f + 3\Delta$ form another QC, and broadcast a new block, $B'$ to all of the honest replicas. These
$n-f$ honest replicas receive this block within $T_f + 4\Delta$, and will see two QCs in 
consecutive views, and will therefore commit the block proposed in $v$.
If $v''>v'+2$, the leader will receive $n-f$ \textsc{Vote-REQ} 
messages that extend $B'$ after $T_f$. Since the leader of $v'+1$ honest, the
highest \textsc{Vote-REQ} that the leader receives will be for a block that extends $B'$. Even
though there may be equivocation, it will only be for a child block of $B'$, and therefore extend
$B$. The leader of $v''$ will
then certify at least $B'$, and send a \textsc{Vote-REQ} containing this QC to all honest replicas, who will commit $B$ after $T_f + \Delta$, since $v'$ and $v'+1$ are in consecutive 
views. 
\end{proof}

%liveness argument:
%let v and v' be two views with honest leaders after GST, and there is no equivocation then
%block B will be committed, in v' leader of v' will see common prefix of 2f+1 pre-prepares
%for B and will be able to form a lock, even if there are many different extensions of B.
%Basically need to prove by induction that for every view between v and v' that 2f+1 honest
%will update their pp to be for B or an extension of B, then in v' after waiting delta v'
%will see 2f+1 honest with common prefix for B and thus will be able to certify it 
%
%leader of v will propose B, since no equivocation B will be highest pp, v+1 has to certify
%but no
%
%
%let v and v' be two view with honest leaders after GST. in v' either a block that
%extends B will be certified
%or an equivocation proof would have formed.
%
%from v to v' n-f honest will have pre-prepare for B or they will update their pre-prepare
%to extend B and have a QC for B, why? because once n-f honest have pre-prepare for B in v' leader will wait delta so n-f votes can form a
%QC for B and then after another delta all n-f honest will have QC for B, or if n-f don't have
%pre-prepare then there must be at least one that has a QC for B, which will be the highest
%and after another delta they will update their $QC_r$ to be for B
%
%also since leader of v is honest we know that it cannot equivocate, therefore in in v+1 the
%exclusive highest pre-prepare must be for B,
%
%in view v, leader of v will receive n-f QCs and n-f pre-prepares, and compute highQC and
%highPP. If highQC.v = v-1, then it is highest possible lock so no way there could be
%a conflicting hidden lock. If highQC.v != v-1 but there are no conflicting pre-prepares > 
%highQC.v then also proof of no conflicting hidden lock. If there is a conflicting
%pre-prepare in view v the
%
%after 3 delta n-f honest will receive and update their preprepare to B, and then for every
%view until v' they will update their preprepare to be for a block that extends B
%
%issue is that n-f honest will all have pp that extend B but may be for different blocks,
%so B cannot be certified
%change certify rule to look at chain of parents for pp, and if there are $n-f$ for a block in 
%same view then certify
%
%
%v and v' views with honest leaders after GST, in view v honest will propose B and n-f honest
%will have pp for B, then a malicious leader is forced to send pp that extends B. A malicious
%leader can equivocate to have two different pp that extend B

%\begin{lemma}\label{lem2}
%If an honest replica $r$ commits a block $B$ in view $v$ after receiving $QC_B$,
%then there exists no quorum certificate for a block that conflicts with $B$ in a view $v'$, 
%s.t. $QC_B.B.QC.v < v' < QC_B.v$.
%\end{lemma}
%
%\begin{lemma}
%If in view $v$, there exists a \textsc{Pre-Prepare}, $pp$, that does not extend $highQC.B$ then
%there must have been equivocation in $pp.v$.
%\end{lemma}
%
%\begin{proof}
%Since $highQC$ formed, this implies $f+1$ honest replicas have a \textsc{Pre-Prepare} in view
%$highQC.B.v$. Thus in view $highQC.B.v+1$ there must be 
%\end{proof}
%
%\begin{lemma}
%If a block $B$ is certified then for every view after $v' > B.v$ the highest 
%\textsc{Pre-Prepare} must be for a block that extends $B$.
%\end{lemma}
%
%\begin{proof}
%We prove the lemma by induction.
%
%\par \textbf{Base Case: v'=B.v+1}. If $B$ is certified this means that $f+1$ honest replicas
%have a \textsc{Pre-Prepare} for $B$ in view $B.v$. This intersects the view change quorum
%of view $B.v+1$ in at least $1$ honest replica, which has this \textsc{Pre-Prepare} in view
%$B.v$, which is the highest possible view for a \textsc{Pre-Prepare}.
%
%\par \textbf{Step.} Before broadcasting a proposal $B'$, $B'$ must extend the highest
%\textsc{Pre-Prepare} that extends the highest QC in the view change. If the view of the
%highest QC is in view $v^*$ and the current view is $v$ then there cannot be a conflicting 
%\textsc{Pre-Prepare} between $v^*$ and $v$ because otherwise there could exist a
%conflicting QC between $v^*$ and $v$
%
%We assume the lemma holds for all $v'-1 > B.v$, and now we consider view
%$v'$. In view $v'-1$ the highest \textsc{Pre-Prepare} must be for a block that extends $B$.
%It must extend $highQC$, since if it did not then by lemma 1 there must have been a detectable
%equivocation.
%\end{proof}
%
%\begin{lemma}
%If an honest replica $r$ commits a block $B$ that was certified in view $v$ then there must
%exist at least $f+1$ honest replicas that have a $pp_r$ for a block that extends $B$ for all
%views $v'>B.v$.
%\end{lemma}
%
%\begin{proof}
%Proof by induction
%
%\par \textbf{Base Case: v'=B.v+1}. Since $B$ was certified there must be $f+1$ honest that
%set $pp_r$ to $B$.
%
%\par \textbf{Step}. We assume lemma holds for all $v'-1>B.v$, now we consider view $v'$.
%From the induction hypothesis it must be the case $f+1$ honest replicas have a $pp_r$ that
%extends $B$ which intersects the view change quorum in $v'$ in at least one honest replica.
%
%\end{proof}
%
%\begin{theorem}
%If an honest replica $r$ commits a block $B$ that was certified in view $v$, then every QC
%formed in view $v'>v$ must be for a block that extends $B$.
%\end{theorem}
%
%\begin{proof}
%We prove the theorem by cases. Let $QC_B$ be the QC that certifies $B$ and let $QC_{B*}$ be
%the QC that causes $r$ to commit $B$.
%
%\par \textbf{Case $QC_B.v < v' < QC_{B*}.v$}. If $QC_B$ formed then $f+1$ honest
%replicas must have a valid \textsc{Pre-Prepare} in view $B.v$ and a proof that this
%\textsc{Pre-Prepare} was the highest in $B.v$. In order for $QC_{B'}$ to form it must have
%been the case that in $v'$ the highest \textsc{Pre-Prepare} did not extend $B$. This can
%only occur if between $B.v$ and $v'$ there exists at
%
%\par \textbf{Case $QC_B.v < v' < QC_{B*}.v$}. Assume for the sake of contradiction that a QC,
%$QC_{B'}$, formed in view $v'$ for a conflicting block $B'$. This implies that a quorum
%$Q'$, s.t. $|Q'|=n-f$ voted for $B'$ in view $v'$. In $v'$, every replica in $Q$ must have 
%updated its local $pp_r$ to be a valid \textsc{Pre-Prepare} message containing $B'$. Let
%$v^*$ be the first view $> v'$ for which a block $B^*$ is a parent of the chain ending with
%$QC_{B*}.B$. 
%\end{proof}
%
%\begin{theorem}
%If an honest replica $r$ commits a block $B$ from seeing a QC formed in view $v$, then every QC
%formed in view $v'>v$ must be for a block that extends $B$.
%\end{theorem}
%
%\begin{proof}
%We prove the theorem by induction on view $v'$.
%
%\par \textbf{Base Case:} Let $v'=v$. From lemma ~\ref{lem1}, there can be at most one QC in a 
%view, and since there is a QC that extends $B$ for view $v$, there cannot be a another 
%conflicting QC that forms in view $v$.
%
%\par \textbf{Step:} We assume the theorem holds for all $v'-1>v$, and now consider $v'$.
%Suppose for the sake of contradiction a conflicting $QC'$ formed in view $v'$. Since $r$
%committed $B$ from receiving a $QC_B$ formed in view $v$ it must be the case that $f+1$
%honest replicas have a $QC_r.B=B$ or by lemma ~\ref{lem2} have a $QC_r$ that extends $B$.
%Let this quorum of $f+1$ honest replicas be $Q$.
%
%In the view change of view $v'$, the leader received QCs from $2f+1$ replicas. Let this quorum
%be $Q'$. It must be the case that the leader had a $highQC$ for
%$QC'.B$, since $QC'$ formed in $v'$. Since all QCs formed in views $\geq QC_B.B.QC.v$ must be 
%for a block that extends
%$B$, it must be the case that $highQC$ has a view $< QC_B.B.QC.v$. However, $Q \cap Q'$ in
%at least one honest replica who has a $QC_r$ with view at least $\geq QC_B.B.QC.v$, a
%contradiction.
%\end{proof}


==> podc_2022/pseudocode.tex <==
\section{Pseudocode}
\label{pseudocode}
We summarize protocol pseudocode. By convention, we assume that each replica only ever accepts messages 1) whose signatures are valid 2) in matching views. We omit this check for clarity. 

\begin{algorithm}

\begin{algorithmic}
\Event {2f+1 \msg{VOTE-RESP}{B_{v-1}}}
\State{$b_h$ = set of submitted client operations}
\State{Form $QC_B = (B_{v-1}, B.v, \mbox{2f+1 VOTE-RESP msgs})$}
\State {$h = B_{v-1}.h + 1$}
\State {$B=(h, H(B_{v-1}), b_h, v, QC_B, \sigma_L)$ where $\sigma_L$ is leader's signature and v the current view}
\State{Send \msg{VOTE-REQ}{B}}
\EndEvent
\Event{\msg{VOTE-REQ}{B}}
\If{$vp_r.v < B.v \land B.QC.v = v_r-1$}
\State{$vr_r$ = \msg{VOTE-REQ}{B}}
\State{$QC_r = B.QC$}
\State{Send \msg{VOTE-RESP}{B}$_{\sigma_r}$ to $L_{v+1}$}
\State{$vp_r$ = \msg{VOTE-RESP}{B}}
\State{$v_r = v_r+1$}
\Else 
\State{Ignore message}
\EndIf
\EndEvent
\end{algorithmic}

\caption{Fast-View Change}\label{fast:vc}
\end{algorithm}


\begin{algorithm}

\begin{algorithmic}

\Event{View $v-1$ timeout expiring}
\State{Send \msg{NewView}{v, vr_r, vp_r, QC_r}$_{\sigma_r}$ to $L_v$}
\EndEvent

\Event{S = 2f+1 \msg{NewView}{v, vr_r, vp_r, QC_r}}\label{leaderlogic}
\If {$2f+1$ matching $vp_r$}
\State $QC_i = $ set of matching $vp_r$
\Else
\State $B_{anc} = $ earliest ancestor block of $2f+1$ matching $vp_r$
\If {$B_{anc}$ uncommitted}
\State $QC_{anc} = $ set of matching $vp_r$
\Else
\State $QC_{high} = max(QC_r)_{r \in R}$
\State $QC_{choice} = max(QC_i, QC_{anc}, QC_{high})$
\State{$highVote = max(vr_r)_{r \in R}$}

\If {$QC_{choice} \longleftarrow highVote.B$}
\Comment{highVote is the correct block to extend}
\Else
\If{$highVote.B.S$ contains $n-f$ \textsc{NewView} messages that do not contain $QC_{choice}$}
\Comment{$QC_{choice}$ could not have committed}
\State $QC_{choice} = highVote.QC$
\Else
\State{$highVote = vr_r$ that contains $QC_{choice}$}
\EndIf
\EndIf
\EndIf
\EndIf
\State{$b_h = $ batch of transactions}
\State{$votereqs = $ set of $vr_r$ messages with the same view $vr_r.B.v$ but different $vr_r.B$}
\If{$votereqs \neq \bot$} \Comment{Equivocation proof}
\State{$\pi = votereqs$}
\EndIf
\State{$B = (h, H(highVote.B), b_h, v, QC_{choice}, S, \pi)$}
\State{$\sigma_{L_v} = $ signature on $B$}
\State{Multicast \msg{Vote-REQ}{B}$_{\sigma_{L_v}}$ to all replicas}
\EndEvent

\Event{\msg{VOTE-REQ}{B}}
\If{$v == B.v$}
\If{$B.\pi \neq \bot$}
\State{Ignore messages from identified faulty leader}
\EndIf
\State{\textbf{goto} line~\ref{leaderlogic} using $B.S$} \Comment{Check if the leader did the view change correctly}
\If{result matches $B$}
\State{$vr_r$ = \msg{VOTE-REQ}{B}}
\State{$QC_r = B.QC$}
\State{Send \msg{VOTE-RESP}{B}$_{\sigma_r}$ to $L_{v+1}$}
\State{$vp_r$ = \msg{VOTE-RESP}{B}$_{\sigma_r}$}
\State{$v_r=v_r+1$}
\Else
\State{Ignore message}
\EndIf
\Else
\State{Ignore message}
\EndIf
\EndEvent
\end{algorithmic}

\caption{Slow View Change}\label{slow:vc}
\end{algorithm}


==> podc_2022/pseudocode_final_commit_rule.tex <==
\begin{algorithm}

\begin{algorithmic}

\Event{Updating $vr_r$}
\State{$QC_r = vr_r.QC$}
\State{$B_r = QC_r.B$}
\State{$QC_{commit} = B_r.QC$}
\State{$B_{commit} = QC_{commit}.B$}
\If{$B_{commit}.v + 1 == B_r.v$} \Comment{Contiguous QCs}
\State{Commit $B_{commit}$}
\Else
\State{$B^* = B_r$}
\While{$B^*.v \geq B_{commit}.v$}
\State{$reqs=B^*.S$}
\For{$vr \in reqs$}
\If{$vr.B$ extends $B_{conflict}$, where $B_{conflict}.S$ contains \msg{Vote-Req}{B_{commit}} and equivocation proof for $B_{commit}.v$ }
\State{\Return False} \Comment{Cannot commit $B_{commit}$ was proposed by faulty 
leader}
\EndIf
\EndFor
\State{$B^*=B^*.parent$}
\EndWhile
\State{Commit $B_{commit}$}
\EndIf
\EndEvent
\end{algorithmic}

\caption{Commit Rule}\label{commit:rule}
\end{algorithm}

==> podc_2022/related_work.tex <==
\section{Related Work}
\label{sec:related}
\nc{We actually say almost all of it in the background section. Would we not merge? We could have a "3.2": }
Existing BFT protocols can broadly be placed in three categories: stable leader protocols, chained LSO protocols, and partially synchronous protocols with asynchronous fallbacks.

\par \textbf{Stable-Leader.} Traditional 
stable leader protocols such as PBFT \cite{castro1999pbft} protocol and its many derivatives (Zyzzyva~\cite{kotla10zyzzyva}, Aardvark~\cite{aardvark}, SBFT~\cite{gueta2019sbft}, among others \cite{xft}~\cite{cachin2011paxos}) follow a primary/backup structure and require expensive view change mechanisms when leader failures do occur. 
\par \textbf{CLSO.} Recent blockchain-focused  chained BFT SMR systems (most notably Hotstuff~\cite{yin2019hotstuff}, Casper FFG~\cite{buterin2017casper} and Tendermint~\cite{buchman2016tendermint}) \nc{Add fast hotstuff, wendy, and Jolteon?} instead move view changes onto the critical path of the protocol and rotate leaders preemptively. Such protocols improve fairness by spreading proposal responsibility evenly across replicas. They are frequently engineered to utilize signature aggregation schemes to achieve linear word complexity. Recent, more optimized variants (DiemBFTv4~\cite{diem2021}, Fast-Hotstuff~\cite{jalalzai2020fasthotstuff}, Jolteon~\cite{jolteon-ditto}) have gone back on this decision and favor more expensive solutions communication-wise, but with fewer number of rounds.
\sys{} also minimizes the number of rounds necessary to commit an operation, but relaxes the commit rule to achieve better performance under failures. 
\par \textbf{Asynchronous Fallback.} When network conditions or failures prevent blocks from
being committed other BFT-SMR protocols like Ditto~\cite{jolteon-ditto}, Dumbo-Bolt 
Transformer~\cite{dumbo-transformer}, and Bullshark~\cite{bullshark} explicitly combine partially synchronous
and fully asynchronous BFT-SMR protocols.
In the common failure-free case, these systems follow a partially synchronous protocol but fallback to an
asynchronous protocol run when failures occur or the network is poor. While the
asynchronous fallback mechanism improves robustness, it also increases commit latency significantly. Additionally, there are fully asynchronous protocols such as HoneyBadgerBFT~\cite{honeybadger},
BEAT~\cite{beat}, VABA~\cite{vaba}, DAG-Rider~\cite{dag-rider}, and more ~\cite{cachin-atomic-broadcast}~\cite{cachin-random-oracles}. While these protocols
are more robust compared to partially synchronous protocols, they typically have higher communication complexity and latency.

\par \textbf{Leader Election Schemes.} Carefully optimizing the leader-selection process for \sys{} is an
orthogonal line of research that could benefit~\sys{} or any CLSO protocol. Rather than having a simple round-robin assignment of
leaders to views, protocols like Carousel~\cite{carousel} implement a leader reputation scheme to detect
and avoid potentially crashed leaders. This increase the probability that $k$ consecutive
honest leaders are elected. \changgebars{}{Carousel guarantees an honest block is committed in $O(f)$ rounds, whereas in $O(f)$ rounds we get $x$ blocks committed and $y$ equivocation detections, where $x+y=O(f)$.} \fs{don't think the detail is necessary here} \fs{could add prosecutor ref and just say it makes it hard to be elected unless you are making progress}
%:-- different leader election schemes:  basic: Round robing and random. 
%:    advanced: Carousel: 
%:              Prosecutor: Raft-like leader election (replicas propose themselves), but usesincreasing PoW to make it hard to elect often -- threshold lowers if leader commits a lot
%:              
%-- all of these are safe during asynchrony, but guarantee liveness only during sufficiently long periods of synchrony.


%-- there is also a class of fully asynchronous protocols such as Honeybadger -- rely on randomization to sidestep flp
%-- some existing work combines partial sync and async: partially sync common case protocol; fallback to async protocol when network is poor. Async provides robustness, but increases commit latency. (Narwahl and Tusk, Bullshark)

%-------------------------\fs{ old version starts here}
%
%\par \textbf{Asynchronous Fallback.} When network conditions or failures prevent blocks from
%being committed other BFT-SMR protocols like Jolteon/Ditto, Dumbo-Bolt 
%Transformer, and Bullshark take a different approach by combining partially synchronous
%and fully asynchronous BFT-SMR protocols.
%They have a partially synchronous protocol run in the common case but fallback to an
%asynchronous protocol run when failures occur or network conditions are not good. While the
%asynchronous fallback provides increased robustness, it increases commit latency significantly.
%
%\par \textbf{Leader Election Schemes.} Instead of having a simple round-robin assignment of
%leaders to views, other protocols like Carousel adapt a leader reputation scheme of detecting
%and avoiding potentially crashed leaders to increase the probability that $k$ consecutive
%honest leaders are elected. This approach is orthogonal to our work, and we can adapt it
%to our protocol to have better performance. Carousel guarantees an honest block is committed
%in $O(f)$ rounds, whereas in $O(f)$ rounds we get $x$ blocks committed and $y$ equivocation
%detections, where $x+y=O(f)$.
%
%\par \textbf{Chained Leader Speaks Once (CSLO) Protocols.} Tendermint was the first protocol
%to bring blockchain style chaining to classical BFT-SMR protocols. While it had leader rotation
%and chaining, it was not a CSLO protocol since the leader was not rotated immediately after
%broadcasting a proposal. Casper FFG, was the first CSLO protocol but lacked optimistic
%responsiveness. HotStuff further popularized CSLO protocols, and improved on prior work by
%adding optimistic responsiveness and a linear view change protocol. Newer CSLO protocols such
%as DiemBFTv4, Fast-HotStuff, and Jolteon, eschew the linear view change of HotStuff for a 
%reduction in latency, since anyway the view synchronization mechanism must be quadratic. All
%of these protocols have a \textit{strict commit rule} in that they can only commit if QCs form
%in consecutive views.
